Quest for a solution to drift in phase change memory devices

The goal of this thesis is to gain new insights into the drift phenomenon and identify strategies to mitigate it. An extensive experimental characterization of PCM devices and in particular drift forms the foundation of each chapter. With respect to time-scales, ambient temperature, device dimensions, and combinations thereof, drift is studied under unprecedented conditions. In three studies, different aspects of drift are examined. (1) The origin of structural relaxation: Drift measurements over 9 orders of magnitude in time reveal the onset of relaxation in a melt-quenched state. The data is used to appraise two models, the Gibbs relaxation model and the collective relaxation model. Additionally, a refined version of the collective relaxation model is introduced and the consequences of a limited number of structural defects are discussed. (2) Exploiting nanoscale effects in phase change memories: Scaling devices to ever-smaller dimensions is incentivized by the requirement to achieve higher storage densities and less power consumption. Eventually, confinement and interfacial effects will govern the device characteristics. Anticipating these consequences, the feasibility to use a single element, Antimony, is assessed for the first time. The power efficiency, stability against crystallization, and drift are characterized under different degrees of confinement. (3) State-dependent drift in a projected memory cell: New device concepts are aiming to reduce drift by decoupling the cell resistance from the electronic properties of the amorphous phase. A shunt resistor scaling with the amount of amorphous material is added. Simulations and the drift characteristics of a projected device put the idealized concept to the test. The contact resistance between the phase change material and the shunt resistor is identified as a decisive parameter to achieve the desired device properties.

==> chapters/Summary_long.tex <==
\chapter{Summary}

Phase change memory (PCM) is an electronic memory technology. In a phase change memory device, switching between a crystalline and amorphous material state occurs in nanoseconds and is thermally induced by Joule heating. The resistivity contrast between the two material states allows information to be encoded. Dependent on the amount of low resistive crystalline and high resistive amorphous material, a quasi-analog resistance can be programmed into the device. This multi-level storage capability could give PCM the edge compared to other more established technologies. Additionally, it makes PCM suitable for in-memory computing. By executing certain computational tasks in the memory, this non-von Neumann computing paradigm aims to reduce the amount of data that needs to be shuttled between the processing (CPU) and memory unit (DRAM). Multi-level storage, however, is impeded by a continuous increase of the amorphous state's resistivity. This phenomenon, called drift, remains one of the most pressing issues of PCM technology. To date, only binary PCM chips have been productized.

The goal of this thesis is to gain new insights into the drift phenomenon and identify strategies to mitigate it. An extensive experimental characterization of PCM devices and in particular drift forms the foundation of each chapter. With respect to time-scales, ambient temperatures, device dimensions and combinations thereof, drift is studied under unprecedented conditions. In three studies, different aspects of drift are examined.

\textbf{Study 1 - The origin of structural relaxation:} Drift has been attributed to structural relaxation of the non-equilibrium amorphous state created by melt-quenching. Models predict that it takes a certain amount of time before the thermally activated structural relaxation processes begin. We employ the threshold switching voltage (\Vth{}) as a means to observe the state of relaxation. These drift measurements at ambient temperatures between \unit[100]{K} and \unit[300]{K} over 9 orders of magnitude in time reveal the onset of relaxation in a melt-quenched device state. The data is used to appraise two phenomenological models for structural relaxation, specifically the Gibbs relaxation model and the collective relaxation model. Additionally, a refined version of the collective relaxation model is introduced and consequences of a limited number of structural defects are discussed.  

The evolution of \Vth{}, between \unit[$\sim$30]{ns} and \unit[10]{s} after melt-quenching the device, exhibits three distinct regimes. Initially, within the first $\mu$s \Vth{} increases steeply, next the value stagnates and finally begins to increase again proportional to log(t). We attribute regime 1 to the decay of the RESET excitation (electronic and/or thermally) and identify the dynamics of structural relaxation as the cause of regimes 2 and 3. The shift of the transition between these regimes with temperature is captured by the Gibbs model and the collective relaxation model. The excellent match between experimental data and the models can be considered another indication that drift in phase change materials must be attributed to structural relaxation.  

Regarding the limitations and potential shortcomings of the Gibbs model, it should be noted that a uniform defect distribution appears to capture the experiments best. The sensibility of such a distribution, in particular across all kinds of materials exhibiting a log(t)-dependent change of their physical properties, has been questioned frequently. Additionally, our Monte Carlo simulations of a system with a fixed number of defects show that in this scenario resistance drift would probably exhibit step-like jumps. We conclude that the relaxation of one defect must be expected to create new defects that relax later. The defect spectrum used in the Gibbs model to describe the relaxation does not exist at any time but is actually the result of an integration of defects that limit the further progress of relaxation over time.

Both relaxation models must be modified if structural relaxation is facilitated by many-body thermal excitation. Here, we discussed the implications for the collective relaxation model. Within the studied temperature range, both versions of the model capture the experiments with subtle differences. At even higher temperatures $\sim$\unit[350]{K} and above, however, the model predictions begin to deviate. As k\textsubscript{b}T approaches the energy of a single excitation process, the modified model predicts a significantly larger threshold voltage drift coefficient and a weaker temperature dependence of the relaxation onset. As long as the phase change material does not begin to crystallize, drift measurements at higher temperatures could allow differentiating which model prediction is correct; an essential step to identifying a model that allows simulating reliably the impact of time, but also temperature variations on \Vth{} and device resistance.  
\newpage
\textbf{Key findings:}
\begin{itemize}
	\item	In a \GST{} mushroom cell, the onset of structural relaxation is around \unit[$\sim$15]{$\mu$s} after melt-quenching the device, at \unit[300]{K} ambient Temperature. At this time, defects with activation energy on the order of \unit[150]{meV} begin to relax. 
	
	\item	Assuming a fixed, finite number of defect states is created during melt-quenching and vanishes upon relaxation cannot plausibly explain drift in phase change materials. Instead, the relaxation of a structural defect must be expected to result in another defective configuration that can relax further. The collective relaxation model is motivated by this very idea. In this regard, the defect distribution defined in the Gibbs model is misleading. 
	
	\item	We have shown how the Meyer-Neldel rule can be incorporated into the collective relaxation model. If structural relaxation is enabled by thermal many-body excitations, as other studies indicate, this refined model should be used to describe drift. Both versions of the model capture the experimental data, but for higher ambient temperatures the model predictions begin to deviate notably. 
\end{itemize}

\textbf{Study 2 - Exploiting nanoscale effects in phase change memories:} Scaling devices to ever-smaller dimensions is incentivized by the requirement to achieve higher storage densities and less power consumption. Eventually, confinement and interfacial effects will govern the device characteristics, not the bulk properties of the phase change material. Anticipating these consequences, the feasibility to use a single element is assessed for the first time. In the devices, pure Antimony is confined one-dimensionally in the range from $\sim$9 atomic layers (\unit[3]{nm}) to $\sim$30 atomic layers (\unit[10]{nm}). Efficient heat dissipation and abrupt ending of the electrical excitation proved to be instrumental parameters to change the device temperature by hundreds of kelvins within nanoseconds, sufficiently fast to avoid complete recrystallization of the molten volume. 

The power efficiency, stability against crystallization and drift are characterized under different degrees of confinement. One-dimensional confinement of the Sb through a thickness reduction does not alter the resistance drift coefficient, but it improves the device efficiency and increases the stability against crystallization by orders of magnitude. We note that the metric for the stability against crystallization defined here only gives an estimate for how long two states (SET and RESET) can be distinguished. Thus, it should at best be considered a very optimistic estimate of the achievable retention times. Nevertheless, it is worth noting that the crystallization time of the \unit[3]{nm} Sb sample (\unit[32]{s} at \unit[80]{$^\circ$C}) already exceeds the DRAM refresh interval by 500x \cite{JEDEC2003} whereas the \unit[10]{nm} sample could not even be amorphized at room temperature. An additional improvement of the stability against crystallization could be achieved by a further well-controlled reduction of the thickness or the use of other cladding materials. Recently published experiments by Cheng et al. indicate that optically melt-quenched Sb (\unit[3]{nm}), sandwiched between indium-tin-oxide might be more stable against crystallization \cite{Cheng2021}.  

We would like to highlight three consequences of this work for future research and device optimization. 

First, with ongoing device scaling interfacial and confinement effects will eventually outweigh bulk material properties. Instead of tuning phase change material compositions, the optimization of device properties can be achieved through the careful engineering of interfaces. To this end, a better understanding of how phase change material properties vary near different interfaces, e.g., due to their atomic-scale roughness, rigidity, nature of the chemical bond, or mechanical strain, is required. Quantitative analyses in theory, simulations, and experiments studying these dependencies under careful control of all mentioned aspects are lacking. Our work demonstrates the impact such research could have for realizing reliable phase change-based devices integrated with the highest spatial density. 

Second, the simplest material imaginable, a pure element, can become a viable alternative to established phase change materials when confined in extremely small volumes. In principle, any material must be expected to exhibit some resistivity contrast between crystalline and amorphous phase. Other elements, besides Sb, could also be suitable for PCM devices. In particular, As has been identified as a potential candidate \cite{Suhrmann1939,Kooi2020}. Resistive switching with a relatively small contrast between crystalline and amorphous phase (\textless 2x) has been reported for devices based on two metallic glass formers, Ta and Mo \cite{Nakanishi2019,Nakanishi2019a}. 

Third, with Sb, we add yet another material to the list of phase change materials exhibiting resistance drift. It must be stressed, once again, that structural relaxation is inherent to the glass state and there seems to be no good reason to assume it will not reflect on the electronic band structure. To suppress drift one must face the challenging endeavor of designing a material in which the density and mobility of free charge carriers do not change, despite a changing band structure. Additionally, we have seen that material confinement neither eliminates nor notably suppresses drift, at least in pure Sb. In the light of these findings, novel device concepts appear to be one of the most promising approaches to mitigate resistance drift. 

\textbf{Key findings:}
\begin{itemize}
	\item	Melt-quenched amorphous Sb exhibits the same characteristic properties as established phase change material compounds, namely semiconducting transport, a resistivity orders of magnitude higher than the crystalline phase, threshold switching and drift.
	
	\item	Material confinement improves the robustness against crystallization by orders of magnitude. Still, the Sb must be melt-quenched within a few nano-seconds to create an amorphous state, indicating that confinement might have a much weaker impact on crystal growth in the temperature regime of fast crystallization.
	
	\item	While confinement stabilizes the amorphous phase significantly against crystallization it has no notable impact on the resistance drift coefficient. Interestingly, a rearrangement to the crystalline structure is hindered, but drift, which also results from atomic rearrangement, appears not to differ.
	
\end{itemize}

\textbf{Study 3 - State-dependent drift in a projected memory cell:} New device concepts are aiming to reduce drift by decoupling the programmed device resistance from the electronic properties of the amorphous phase. To this end,
the phase change material is deposited on an electrically conducting material in the projected memory cell. It functions as a shunt resistor that scales with the amount of amorphous material. The resistance drift is suppressed because only a fraction of the read current flows through the amorphous phase change material.

Simulations with an equivalent circuit model and measurements over 7 orders of magnitude in time reveal that drift becomes time and state-dependent in a projected device. The increasingly stronger drift suppression with time is inherent to the projected memory and can be considered a desirable effect. Whereas the state dependence causes a gradual loss of information with time, that cannot be recovered. Since resistance drift exhibits variability anyway (inter but also intra device), the overall drift reduction by projection is  expected still to be beneficial. Furthermore, the drift coefficient only becomes state-dependent if the current flow from the phase change material into the projection layer is hindered. Thus, it is critical to minimize the contact resistivity between the two materials. 
 
As a next step to refine the model and improve its predictive character a more elaborate characterization of \Rint{} is required. Separate measurements of the contact resistivity and transfer length could allow \Rint{} to be determined, assuming \Cref{equ:PROJ_TransferLength} can be applied. Potentially, another phenomenological description is required. For example, it could be due to the device geometry or the metal electrodes which are connected to both materials. Furthermore, we assumed an ohmic contact between projection and crystalline phase change material. If a Schottky barrier forms, \Rint{} to the left and right of the amorphous volume is different. Like in the previous chapter, we identify, once again, a good understanding of interfacial and confinement effects essential to develop future devices. Besides the implications for phase transition dynamics, also those on electronic contacts are critical in a projected memory device. 

\textbf{Key findings:}
\begin{itemize}
	\item	We developed a tractable device model to describe the state and time dependence of drift and how the device resistance scales with the size of the amorphous volume. It captures quantitatively the experiments on projected Sb bridge cells. 
	\item	The time-invariant conduction path in parallel with the drifting amorphous phase change material results in a time-dependent drift coefficient in projected memory cells, irrespective of the device type (mushroom or bridge). The more time elapsed after amorphization, the less the device drifts.  
	\item	The drift coefficient also depends on the size of the amorphous volume because of the interface resistance between the Sb and projection material. With increasing interface resistance compared to the resistance of the amorphous volume (i.e., decreasing size), less read current bypasses the amorphous phase. The drift coefficient increases for smaller amorphous lengths. By minimizing the contact resistivity between projection layer and phase change material, a state-dependent drift coefficient can be avoided. 
\end{itemize}


==> chapters/Zusammenfassung_lang.tex <==
\chapter{Zusammenfassung}

Phasenwechselspeicher sind ein elektronisches, resistives Speichermedium. Das Phasenwechselmaterial in diesem resistiven Speicher (Zelle) kann innerhalb von Nanosekunden in einen kristallinen oder amorphen Zustand versetzt werden. Um einen Phasenwechsel zu erreichen wird das Material mittels joulscher W{\"a}rme erhitzt. Der amorphe Zustand hat einen deutlich gr{\"o}\ss eren spezifischen elektrischen Widerstand als die kristalline Phase. Indem man den Anteil des amorphen und kristallinen Materials in der Zelle {\"a}ndert, kann ein quasi analoger Widerstands programmiert werden. Das Potenzial als Multi-Level Speicher genutzt zu werden, k{\"o}nnte Phasenwechselspeichern im Vergleich zu anderen Speichermedien einen Wettbewerbsvorteil verschaffen. Dar{\"u}ber hinaus er{\"o}ffnent es die M{\"o}glichkeit Phasenwechselspeicher im Bereich des In-memory computing zu verwenden. Mit diesem Konzept versucht man einige Schw{\"a}chen der klassischen von-Neuman Computer Architektur zu umgehen. Indem gewisse Rechenoperationen mit dem analogen Speicher ausgef{\"u}hrt werden, kann die Menge der Daten, die zwischen Speicher und Prozessor transferiert werden muss reduziert werden.  

Bislang k{\"o}nnen Phasenwechselspeicher jedoch nur begrenzt als Multi-Level Speicher genutzt werden, da der spezifische Wiederstand des amorphen Zustands kontinuierlich zunimmt. Dieses Ph{\"a}nomen wird als Drift bezeichnet. Die Zunahme des Widerstandes mit der Zeit kann durch die Gleichung $ R = R_0 \cdot (t/t_0)^{\nu_R}$ beschrieben werden. Dabei bezeichnet $R_0$ den Widerstand zum Zeitpunkt $t_0$ und $\nu_R$ den Driftkoeffizienten. Drift stellt eine der gr{\"o\ss}ten Herausforderungen f{\"u}r die Zukunft dieser Technologie dar. Bislang wurden nur bin{\"a}re Phasenwechselspeicher zur Produktreife entwickelt. 

Das Ziel dieser Arbeit ist es, das Ph{\"a}nomen besser zu verstehen und neue Konzepte mit denen Drift unterdr{\"u}ckt oder reduziert werden kann zu untersuchen. Eine sorgf{\"a}ltige experimentelle Untersuchung von Phasenwechselspeichern und insbesondere ihres Drift bildet den Grundbaustein eines jeden Kapitels. In vielerlei Hinsicht wird Drift von Phasenwechselspeichern unter neuen und extremen Bedingungen vermessen. Dies betrifft die Zeitskalen, die Umgebungstemperatur und die Art der Speicherzellen. Die Arbeit ist in drei Studien unterteilt. 

\textbf{Studie 1 - Der Beginn struktureller Relaxation:} Die meisten Theorien gehen davon aus, dass Drift durch die strukturelle Relaxation des amorphen Zustandes hervorgerufen wird. Der durch das Abschrecken aus der Schmelze erzeugte Zustand befindet sich im Nichtgleichgewicht. Relaxationsmodelle sagen voraus, dass es eine gewisse Zeit dauert, bevor thermisch-aktivierte Relaxationen stattfinden. In dieser Studie wird die {\"A}nderung der Spannung, bei der amorphe Zustand einen sprunghaften Anstieg der Leitfaehigkeit aufweist (\Vth), mit der Zeit kann genutzt, um die Relaxation der amorphen Phase zu untersuchen. In diesen Messungen, {\"u}ber 9 Gr{\"o}\ss enordnungen in der Zeit und bei Umgebungstemperaturen zwischen \unit[100]{K} und \unit[300]{K}, kann der Beginn der strukturellen Relaxation beobachtet werden. Die Daten werde genutzt um zwei ph{\"a}nomenologische Relaxationsmodelle, das Gibbs Modell und das Collective Relaxation Modell, zu vergleichen und pr{\"u}fen. Desweiteren wird eine erweiterte Version des Collective Relaxation Modell entwickelt und diskutiert welche Folgen eine begrenzte Anzahl struktureller Defekte f{\"u}r das Gibbs Modell h{\"a}tte.

Die zeitliche {\"A}nderung von \Vth{} zwischen $\sim$\unit[30]{ns} und \unit[10]{s} nach dem Erzeugen des amorphen Zustandes wei{\ss}t drei Abschnitte auf. Zu Beginn, innerhalb der ersten $\mu$s nimmt \Vth{} deutlich zu, anschlie{\ss}end stagniert der Wert und steigt schlie{\ss}lich proportional zu log(t). Wir gehen davon aus, dass der erste Abschitt durch das Abklingen der elektronischen und thermischen Anregung beim Programmieren der Zelle zu erkl{\"a}ren ist. Die Abschnitte 2 und 3 k{\"o}nnen durch die Dynamik der strukturellen Relaxation erkl{\"a}rt werden. Die beobachtete {\"A}nderung von \Vth{} in diesen beiden Abschnitten kann sowohl mit Gibbs Modell, als auch von Collective Relaxation Model reproduziert werden. Dies ist eine weiterer Anhaltspunkt daf{\"u}r, dass Drift in Phasenwechselmaterialien durch strukturelle Relaxation hervorgerufen wird.

Was die Grenzen und M{\"o}gliche Schwachpunkte des Gibbs Modells betrifft, sollte festgehalten werden, dass die Experimente am besten durch eine stetigen Gleichverteilung von strukturellen Defekten beschrieben werden. Die Plausibilit{\"a}t einer solchen Verteilung ist fraglich. Dies gilt insbesondere, weil sie auch erforderlich ist, um eine {\"A}nderung der physikalischen Eigenschaften proportional zu log(t) zu beschreiben, welches in verschiedensten amorphen Materialien zu beobachten ist. Die hier durchgef{\"u}hrten Monte Carlo Simulationen eines Systems mit einer begrenzten Anzahl struktureller Defekte zeigen au{\ss}erdem, dass Drift in diesem Szenario diskontinuierlich erfolgen w{\"u}rde. Daraus l{\"a}sst sich Schlussfolgern, dass die Relaxation eines strukturellen Defekts neue Defekte erzeugt, die zu einem sp{\"a}teren Zeitpunkt relaxieren. Entsprechen existiert die im Gibbs Modell beschriebene Verteilung der strukturellen Defekte zu keinem Zeitpunkt. Statt dessen kann sie als Ergebnis einer Integration der Defekte, die das weitere Fortschreiten der Relaxation behindern, {\"u}ber die Zeit verstanden werden. 

Beide Modelle m{\"u}ssen neu formuliert werden, wenn die energetische Anregung der strukturellen Relaxation durch die Vielteilchentheorie beschrieben wird. In dieser Arbeit werden die Konsequenzen anhand des Collective Relaxation Modell diskutiert. Innerhalb des experimentell untersuchten Temperaturbereiches, unterscheiden sich die beiden Versionen des Modells kaum. Erst f{\"u}r h{\"o}here Temperaturen beginnen die Vorhersagen der Modelle voneinander abzuweichen. Je {\"a}hnlicher \kb T der Energie eines Phonons ist, desto deutlicher weichen die Vorhersagen voneinander ab. Das erweiterte Modell sagt eine st{\"a}rkere Zunahme von \Vth{} durch Drift und eine geringe {\"A}nderung des Beginns der Relaxation mit der Temperatur voraus. Sofern das amorphe Phasenwechselmaterial bei diesen Temperaturen nicht kristallisiert, k{\"o}nnen weitere Experimente helfen festzustellen, welche Version des Modells besser geeignet ist den Drift in Phasenwechselmaterialien zu beschreiben. Dies ist ein wichtiger Schritt um ein universelles Modell zu entwickeln mit dem die {\"A}nderung von \Vth{} und dem elektrischen Widerstand der Zelle beschrieben werden kann. 

\textbf{Wichtige Erkenntnisse:}

\begin{itemize}
	\item	Der amorphe Zustand beginnt bei \unit[300]{K} etwas \unit[$\sim$15]{$\mu$s} nach dem Abschrecken aus der Schmelze strukturell zu relaxieren. Die zuerst relaxierenden Defekte haben eine Aktivierungsenergie von etwa \unit[150]{meV}. 
	
	\item 	Unter der Annahme, dass nur eine begrenzte Anzahl struktureller Defekte existiert, die alle w{\"a}hrend des Abschreckens aus der Schmelze eingefroren wurden, kann Drift in Phasenwechselmaterialien nicht plausibel erkl{\"a}rt werden. Statt dessen ist davon auszugehen, dass die Relaxation eines Defekts neue Defekte generiert, die weiter relaxieren k{\"o}nnen. Diesbez{\"u}glich ist die im Gibbs Modell verwendete Verteilung von strukturellen Defekten missverst{\"a}ndlich. Das Collective Relaxation Modell hingegen ist durch genau diese Idee motiviert. 
	
	\item 	Es wurde gezeigt, wie das Collective Relaxation Modell um die Meyer-Neldel Regel erweitert werden kann. Andere Studien deuten darauf hin, dass Relaxationsprozesse durch eine Vielzahl von Phononen angeregt wird. In diesem Fall sollte die Meyer-Neldel Regel ber{\"u}cksichtigt werden. Mit beide Versionen des Modells k{\"o}nnen die Experimente reproduziert werden. Erst bei einer Extrapolation zu h{\"o}heren Temperaturen beginnen sich die Vorhersagen zu unterscheiden. 
\end{itemize}

\newpage
\textbf{Studie 2 - Wie sich Effekte im Nanobereich nutzen lassen:} Um h{\"o}here Speicherdichten und eine bessere Energieeffizienz zu erreichen ist es erforderlich elektronische Speicher in immer kleineren Dimensionen zu bauen. Entsprechend werden die Eigenschaften eines Phasenwechselspeichers irgendwann durch Grenzflächeneffekte dominiert werden und nicht mehr nur von den Eigenschaften des Phasenwechselmaterials abh{\"a}ngig sein. Im Anbetracht der zu erwartenden Folgen stellt sich die Frage, ob anstelle der etablierten Chalcogenid Legierungen auch ein reines Element in Phasenwechselspeichern genutzt werden kann. In den hier untersuchten Zellen wird pures Antimon mit Schichtdicken zwischen \unit[3]{nm} und \unit[10]{nm} als Phasenwechselmaterial eingesetzt. Durch schnelles Abf{\"u}hren der W{\"a}rme und ein abruptes Ende der elektrischen Pulse, durch die das Antimon geschmolzen wird, gelingt es die Temperatur innerhalb von Nanosekunden um mehrere \unit[100]{K} zu senken. So ist es m{\"o}glich amorphes Antimon in den Zellen zu erzeugen. 

Anschlie{\ss}end wurde die Energieeffizienz, Stabilit{\"a}t des amorphen Zustandes gegen Rekristallisation und Drift von Zellen mit unterschiedlichen Antimon Schichtdicken verglichen. Der Driftkoeffizient {\"a}ndert sich nicht. Aber die Zellen werden mit abnehmender Schichtdicke effizienter. Au\ss erdem nimmt die Stabilit{\"a}t gegen Rekristallisation um mehrere Gr{\"o}ssenordnungen zu. Die hier verwendete Metrik dient lediglich der Absch{\"a}tzung wie lange zwei Zust{\"a}nde in der Zelle unterschieden werden k{\"o}nnen (kristallin und amorph). Entsprechend sollte es bestenfalls als eine optimistische Absch{\"a}tzung der maximalen Zeit, die eine Information gespeichert werden kann (Speicherdauer), angesehen werden. Es ist dennoch bemerkenswert das diese Zeitspanne f{\"u}r die \unit[3]{nm} Proben (\unit[32]{s} bei \unit[80]{$^\circ$C}) bereits 500x dem DRAM Aktualisierungsinterval entspricht \cite{JEDEC2003}, wohingegen die \unit[10]{nm} Proben nicht einmal bei Raumtemperatur in einen amorphen Zustand programmiert werden konnten. Eine weitere Verbesserung der Stabilit{\"a}t gegen Rekristallisation k{\"o}nnte mit noch geringeren Schichtdicken oder anderen Materialien an der Grenzfl{\"a}che zum Antimon erreicht werden. Eine vor kurzem ver{\"o}ffentlichte Arbeit von Cheng et al. deutet darauf hin, das Antimon mit einer Zinn-Oxid Grenzfl{\"a}che stabiler gegen Rekristallisation sein k{\"o}nnte \cite{Cheng2021}.

Drei Schlussfolgerungen aus dieser Studie f{\"u}r die Entwicklung und Optimierung zuk{\"u}nftiger Phasenwechselspeicher sollen hervorgehoben werden. 

Erstens, mit der Skalierung zu immer kleineren Dimensionen werden gewinnen Grenzflächeneffekte zunehmend an Bedeutung. Deshalb scheint es ratsam sich in der Forschung zunehmen darauf zu konzentrieren, wie diese Effekte genutzt werden k{\"o}nnen, anstatt Eigenschaften die ein Phasenwechselmaterial moeglicherweise nur in einem gro\ss en Volumen aufwei\ss t zu optimieren. Um dies zu erreichen ist mehr Wissen dar{\"u}ber erforderlich, wie sich beispielsweise die atomare Rauheit, Steifigkeit oder mechanische Spannungen an Grenzflächen auswirken. Quantitative Untersuchungen die dies unter sorgfältig kontrollierten Bedingungen studieren fehlen bislang. Dies betrifft Theorien, Simulationen und Experimente. Die Studie zeigt wie Bedeutungsvoll dieses Wissen f{\"u}r k{\"u}nftige Phasenwechselspeicher sein wird. 

Zweitens, in zu extrem kleinen Dimensionen skalierte Phasenwechselspeicher, k{\"o}nnte das einfachste Material {\"u}berhaupt, ein reines Element, eine alternative zu den etablierten Legierungen darstellen. Es ist davon auszugehen, dass jedes Material einen gewissen Kontrast des elektrischen Wiederstandes zwischen kristalliner und amorpher Phase aufweist. Neben Antimon k{\"o}nnten sich auch andere Elemente f{\"u}r die Anwendung in Phasenwechselspeichern eignen. Beispielsweise Arsen, wurde als potentieller Kandidat identifiziert \cite{Suhrmann1939,Kooi2020}. Bei zwei metallischen Gl{\"a}sern (Tantal und Molybdän) wurde ein relativ kleiner Kontrast zwischen kristalliner und amorpher Phase beobachtet (\textless 2) \cite{Nakanishi2019,Nakanishi2019a}.

Drittens, wie alle anderen bislang untersuchten Phasenwechselmaterialien, weist auch Antimon Drift auf. Strukturelle Relaxation ist ein universales Ph{\"a}nomen in Gl{\"a}sern. Es gibt keinen guten Grund anzunehmen, dass sich diese Relaxation nicht auf die elektronische Bandstruktur auswirkt. Um ein Phasenwechselmaterial zu finden, das nicht driftet, w{\"a}re es somit erforderlich, dass sich diese {\"A}nderungen der Bandstruktur nicht auf die elektrische Leitf{\"a}higkeit auswirken. Au\ss erdem zeigen die Messungen, dass auch das skalieren zu extrem kleinen Dimensionen und Grenzfl{\"a}cheneffekte Drift nicht unterdr{\"u}cken, zumindest in Antimon. Auf Grund dieser Beobachtungen scheinen neue Zellgeometrien der vielversprechendste Ansatz zu sein um Drift zu reduzieren. 

\textbf{Wichtige Erkenntnisse:}
\begin{itemize}
\item 	Das in den Zellen in einen amorphen Zustand versetzte Antimon weist {\"a}hnliche Eigenschaften wie die als Phasenwechselmaterial etablierten Legierungen auf. Der amorphe Zustand ist halbleitend, hat einen um mehrere Gr{\"o}\ss enordnungen h{\"o}heren spezifischen Widerstand, zeigt einen sprunghaften Anstieg der Leitfaehigkeit bei einer kritischen elektrischen Spannung (\Vth) und der elektrische Widerstand driftet. 

\item 	Mit abnehmender Schichtdicke nimmt die Stabilit{\"a}t der amorphen Phase gegen Rekristallisation um mehrere Gr{\"o}ssenordnungen zu. Dennoch ist es erforderlich die Proben innerhalb von Nanosekunden aus der Schmelze abzuschrecken um einen amorphen Zustand zu erzeugen. Dies zeigt, dass der Phasenwechsel bei hohen Temperaturen immer noch extrem schnell stattfinden kann. 

\item  W{\"a}hrend die Stabilit{\"a}t gegen Rekristallisation mit abnehmender Schichtdicke deutlich zunimmt, {\"a}ndert sich der Driftkoeffizient nicht. Die Neuanordnung der Atome in die kristalline Struktur wird zunehmend verlangsamt und behindert. Gleichzeitig bleibt der Drift, welcher aus {\"A}nderungen der atomaren Anordnung innerhalb des amorphen Zustandes folgt, unver{\"a}ndert. 

\end{itemize}

\textbf{Studie 3 - Drift in Projizierten-Zellen:} In der Projizierten-Zelle soll der programmierten Widerstand von den elektronischen Eigenschaften der amorphen Phase entkoppelt werden, um Drift zu reduzieren. Zu diesem Zweck wird das Phasenwechselmaterial auf einem elektrisch leitf{\"a}higen Material deponiert (Projektions-Schicht). Es fungiert als paralleler Widerstand, der mit der gr{\"o}\ss e des amorphen Volumens skaliert. Der Widerstand der Zelle driftet weniger, da nur ein kleiner Teil des elektrischen Stroms beim Auslesen der Zelle durch das amorphe Phasenwechselmaterial fliest. 

Die Analyse eines Ersatzschaltbildes der Zelle und Experimente mit Projizierten-Zellen zeigen, dass sich das Driftverhalten dieser Zellen mit der Zeit {\"a}ndert und von der Gr{\"o}\ss e des amorphen Volumens in der Zelle abh{\"a}ngt. Die mit der Zeit zunehmend st{\"a}rkere Unterdr{\"u}ckung des Drift ist eine w{\"u}nschenswerte Eigenschaft. Die Abh{\"a}ngigkeit von der Gr{\"o}\ss e des amorphen Volumens hingegen f{\"u}hrt dazu, dass Informationen nicht zuverl{\"a}ssig gespeichert werden k{\"o}nnen. Weil der Drift jedoch ohnehin zwischen unterschiedlichen Zellen, aber auch innerhalb einer Zelle variiert, ist die mit dieser Zellgeometrie erreichte Reduktion des Drifts trotz allem von Vorteil. Insbesondere, da die Abh{\"a}ngigkeit von der Gr{\"o}sse des amorphen Volumens nur besteht, wenn der Stromfluss zwischen dem Phasenwechselmaterial und dem parallel angeordneten Widerstand behindert ist. Deshalb ist es besonders wichtig diesen Kontaktwiderstand (\Rint) zu minimieren. 

Um das Modell weiter zu verbessern, ist es erforderlich den Kontaktwiderstand genauer zu bestimmen. Individuelle Messungen des spezifischen Kontaktwiderstandes und der Transferl{\"a}nge w{\"u}rden erlauben \Rint{} zu bestimmen, sofern \Cref{equ:PROJ_TransferLength} g{\"u}ltig ist. M{\"o}glicherweise kann \Rint{} so jedoch nicht berechnet werden. Dies k{\"o}nnte zum Beispiel auf Grund der Geometrie der Zelle der Fall sein, oder weil die Metallelektroden ebenfalls beide Materialien kontaktieren. Desweiteren k{\"o}nnte der Kontakt zwischen dem kristallinen Phasenwechselmaterial und der Projektions-Schicht anstelle eines ohmschen Kontakts ein Schottky-Kontakt sein. 

Wie in der vorherigen Studie wird ersichtlich, dass ein gutes Verst{\"a}ndnis von Grenzfl{\"a}cheneffekten und Effekte im Nanobereich von gr{\"o}\ss ter Bedeutung ist um neue Phasenwechselspeicher zu entwickeln. Neben den Konsequenzen f{\"u}r das Programmieren in einen amorphen und kristallinen Zustand, werden in der Projizierten Zelle auch jene f{\"u}r den Kontaktwiderstand bedeutend. 

\textbf{Wichtige Erkenntnisse:}
\begin{itemize}
	\item 	Es ist m{\"o}glich mit einem einfach zu handhabenden Modell das Driftverhalten einer Projizierten-Zelle in Abh{\"a}ngigkeit von der Zeit und der Gr{\"o}\ss e des amorphen Volumens zu simulieren. Das vorgestellte Modell kann den experimentell gemessen Drift von Projizierten-Zellen quantitativ reproduzieren. Auch das Skalieren des Zellwiederstandes mit der Gr{\"o}\ss e des amorphen Volumens beschreibt das Modell richtig. 
	
	\item	Da der Widerstand der Projektions-Schicht unabh{\"a}ngig von der Zeit ist und nur der amorphe Widerstand driftet, {\"a}ndert sich der Driftkoeffizient in einer Projizierten-Zelle mit der Zeit. Je mehr Zeit vergeht, desto weniger driftet die Zelle. 
	
	\item 	 Auf Grund des Kontaktwiderstandes zwischen Phasenwechselmaterial und Projektions-Schicht h{\"a}ngt der Driftkoeffizient  au\ss erdem von der Gr{\"o}\ss e des amorphen Volumens ab. Je gr{\"o}\ss er der Kontaktwiderstand im Vergleich zum Widerstand des amorphen Volumens ist, also je kleiner das amorphe Volumen ist, desto geringer ist der Anteil des Stroms, der nicht durch das amorphe Volumen flie\ss t. Entsprechend haben kleinere amorphe Volumina einen gr{\"o}\ss eren Driftkoeffizienten. Um diese Ab{\"a}ngigkeit zu verhindern sollte der spezifische Kontaktwiderstand zwischen Phasenwechselmaterial und Projektions-Schicht minimal sein. 
	
\end{itemize}


==> chapters/original1.Projected_Memory.tex <==
\chapter{State-dependent drift in a projected memory cell}
\label{Chapt:Proj}	
% All models are wrong, but some are useful - George Box

\textbf{Preliminary remark:} The results presented in this chapter have been published as a journal article. \newline
1) State dependence and temporal evolution of resistance in a projected phase change memory - Kersting et al. - Scientific reports \cite{Kersting2020} \\[6pt]

The idea of the projected memory is to decouple the device readout from the unstable electrical properties of the amorphous phase. For this purpose, an electrical conducting material, called the projection layer, is placed in parallel to the phase change material. The sheet resistance of the projection layer is chosen to lie between the sheet resistance of the crystalline and the amorphous states of the phase change material. In a projected memory device, the majority of read current bypasses the amorphized volume in the device and flows in the projection layer instead. Hence the resulting device resistance can be viewed as a projection of the length of the amorphous region onto the projection layer. In contrast to the read operation, most current flows through the phase change material during the write operation. When the amorphous phase undergoes threshold switching, its resistance decreases to a fraction of the projection layers' resistance. Like in an unprojected device, the Joule heating required to write the cell is localized inside the phase change material. Ideally, the stable resistance of the projection layer improves the device's memory performance, while the write operation does not change \cite{Redaelli2010,Kim2013,Koelmans2015}. 

In this chapter, a comprehensive device model is developed to capture the behavior of the projected memory bridge cell for any arbitrary device state. Here device state refers to the phase configuration of the phase change material i.e. the amount of crystalline and amorphous volume in the device. We identify the interface resistance between the phase change material and projection layer as a decisive parameter. It hinders the current flow into the projection layer and consequently determines the fraction of read current that bypasses the amorphous volume. Thus, it defines how effectively the projection works. Dependent on the interface resistance, drift characteristics, and scaling of the device resistance with the size of the amorphous volume change significantly. The model is experimentally validated on Sb bridge cells (\unit[3]{nm} thick), both with and without projection layer. Finally, the modeling framework is extended to identify guidelines for materials selection to optimize projected PCM device characteristics.

\section{State of the art}
	
	\subsection{Projected memory - proof of concept}

	Opposed to the amorphous phase change material, a material that exhibits no drift, lower read noise, weaker temperature dependence, and ideally a field-independent electrical transport is chosen for the projection layer. Consequently, drift and read noise reduce by more than one order of magnitude \cite{Kim2013,Koelmans2015}. Additionally, a weak, linear temperature dependence of the resistance has been observed in projected devices, as opposed to the exponential dependence of the amorphous phase change material \cite{Giannopoulos2019}. Last but not least it has been described that projected devices can be recovered after a destructive write (void formation in the phase change material) \cite{Xie2018}. First studies of the ramifications on the in-memory compute performance report significantly improved multiplication accuracy (quantified by the reliability of a single device readout) \cite{Giannopoulos2019} and a slower decay of neural network inference accuracy with time \cite{Bruce2021}. 
	
	Clearly, the proof of concept has been demonstrated. A comprehensive understanding of the device however is still lacking. To guide the design of future device generations a deeper understanding beyond the idealized picture is required. In particular, the interface resistance between phase change material and projection layer must be expected to be finite. Additionally, the resistance ratio between projection layer and amorphous phase changes with time, and the projection efficiency increases. The consequences of these two aspects have not yet been addressed. We also note that to reduce drift and read noise by projection, one must compromise on the dynamic range. It is now defined by the resistance ratio of projection layer and crystalline phase change material. Last but not least it is essential to assess if the resistance drift is state-independent or depends on the size (length) of the amorphous volume.
	
	% Make the connection to the state dependence. 
	
	\subsection{The challenge of state-dependent drift coefficients}

	Among the strategies to mitigate drift, we discussed the idea to rescale the results of the matrix-vector-multiply operation executed with the PCM crossbar array. In the case of resistance independent drift coefficients, this scheme would work perfectly. Since all values (resistances) stored in the crossbar increase by a constant factor the elements of the result vector (column currents) decrease by the same factor. I.e. a global scaling factor could correct drift. In reality, however, drift coefficients vary. Thus, the relative contribution of individual devices to the column current changes with time. For a single matrix column, this variability could still be compensated by row-wise adjusting the read signal. However, since the complete matrix with 'randomly' distributed resistances is multiplied in parallel, the state-dependent drift cannot be corrected perfectly. The global drift correction compensates only the mean drift behavior of the array. The changing relative contribution of individual devices to the column current, due to different drift coefficients, is not corrected and causes a continuous decrease of compute precision with time \cite{LeGallo2018a,Joshi2020}. 
	
	The amorphous phase might exhibit varying drift coefficients. Device-to-device variability for example can result from differences in the local phase change material stoichiometry. Within a single device, the coupling between relaxation and electrical transport might differ in subsequent amorphizations due to the finite size effects. The amorphous volume in the device is so small, that variations in the disordered structure are not averaged out but reflect on the drift. Additionally, the drift coefficient changes depending on the device state i.e. the phase configuration of amorphous and crystalline material in the device. As long as an amorphous volume fills the complete device cross-section the average drift coefficient of an unprojected cell is constant \cite{Kersting2020,GhaziSarwat2021}. This value corresponds to the drift coefficient of the amorphous phase. Intermediate device states exhibit lower drift coefficients. The current path through the device is no longer blocked by a proper amorphous volume. Instead, (crystalline) percolation paths, exhibiting no or much less drift contribute to the device current. With decreasing device resistance the contribution of the percolation path to the device current increases and the drift coefficient decreases to the value of the crystalline state. Typically the crystalline state does not drift. In some doped phase change materials, however, the device SET state has been reported to exhibit drift \cite{Boybat2019,Bruce2021}. It might be caused by the structural relaxation of disordered material at crystal grain boundaries.  
	
	A parallel conduction path to the amorphous phase change material exists in the projected memory cell by design, even when no percolation paths exist in the amorphous volume. However, the resistance ratio between amorphous volume and parallel projection layer remains constant. Thus the projected device is expected to have a constant, yet reduced drift coefficient (when the amorphous volume has no percolation paths). If percolation paths exist in intermediate states, the drift will decrease further. In the scenario of an ideal projected memory cell, both, absolute drift coefficients and their state dependence should be smaller than in an unprojected cell. 
		
	\subsection{Research questions}
	\begin{enumerate}
		\item	Can we design a tractable model of a projected memory bridge cell?
		\item	How do the drift coefficient and device resistance depend on the length of the amorphous volume and the interface resistance between projection and phase change material? 
		\item	How should projection and phase change materials be selected to achieve ideal device characteristics? 
	\end{enumerate}
\newpage
\section{A compact model for projected bridge cells}
	
	In this section, we will introduce the equivalent circuit model for projected bridge cells. With this model, we study the implications of an interface resistance (\Rint) between phase change material and projection layer. Additionally, the equivalent circuit model is compared to FEM simulations and the model input parameters for the projected Sb bridge cell are defined experimentally.    
	
	\subsection{Equivalent circuit model}
	
	For our model of a projected bridge cell, we assume that during RESET the amorphous regions are created close to the center of the device (illustrated in \Cref{fig:PROJ_DeviceModel} a). This has been observed for lateral device structures in both, FEM simulations, as well as TEM studies \cite{Koelmans2015,Castro2007,Goux2009}. Minor shifts from the center of the confined device region can occur due to thermoelectric effects, but such shifts typically remain within the confined region of the device \cite{Castro2007,Oosthoek2015a}. An equivalent electrical circuit of this device during the low-field read operation can be described as a network of resistors, corresponding to the resistances of the crystalline and the amorphous region (\Rc{} \& \Ra) in the device, and the projection layer resistors in parallel to them (\Rprojc{} \& \Rproja). These resistors will be determined by the material’s sheet resistances, the device length (L\textsubscript{line}) and width (w), and the length of the amorphous region (L\textsubscript{amo}) in the device as given by,
	
	\begin{equation}
		R_{cryst} = \frac{1}{2} \cdot R_{s,cryst} \cdot \frac{L_{line}-L_{amo}}{w}
		\label{equ:ProjPCM_Rcryst}
	\end{equation}
	
	\begin{equation}
		R_{proj,c} = \frac{1}{2} \cdot R_{s,proj} \cdot \frac{L_{line}-L_{amo}}{w}
		\label{equ:ProjPCM_Rprojc}
	\end{equation}
	
	\begin{equation}
		R_{amo} = R_{s,amo} \cdot \frac{L_{amo}}{w}
		\label{equ:ProjPCM_Ramo}
	\end{equation}
	
	\begin{equation}
		R_{proj,a} = R_{s,proj} \cdot \frac{L_{amo}}{w}
		\label{equ:ProjPCM_Rproja}
	\end{equation}
	
	Here, \Rsc{} denotes the sheet resistance of the crystalline phase change material, \Rsa{} the sheet resistance of the melt-quenched amorphous phase change material, and \Rsp{} the sheet resistance of the projection material. Additional circuit elements are the contact resistances of the metal electrodes to the projection and phase change material (\RePCM{} and \RePROJ) and the interface resistance (\Rint) between the phase change material and projection layer. These resistors may be non-negligible if a Schottky barrier forms like it has been reported at the interface between amorphous \GST{} and TiN \cite{Huang2014}. Or simply due to the nanoscopic size of the contact. Last but not least the atomic-scale structure (e.g. smooth interfaces, material mixing in an interface layer, or poor adhesion and local delamination) will have an impact on the contact resistance.
	
	\begin{figure}[bth!]
		\centering
		\includegraphics[width=1\linewidth]{figures/PROJ/DeviceModel_Rtotal.pdf}
		\caption{\textbf{Equivalent circuit model of a projected bridge cell.} The projected bridge cell is abstracted to a resistor network. Central building blocks are the crystalline and amorphous resistors with their parallel projection elements. Additionally, we introduce contact resistances to the electrodes. And crucially, an interface resistance between phase change material and projection layer at the crystalline-amorphous interface.}
		\label{fig:PROJ_DeviceModel}
	\end{figure}
	
	Another representation of this resistor network is shown in \Cref{fig:PROJ_DeviceModel}b. With the $\Delta$-Y transformation the $\Delta$ formed by the resistors \RePCM{} + \Rc, \Rint{} and \RePROJ{} + \Rprojc{} (\Cref{fig:PROJ_DeviceModel}a) is translated to a Y formed by R\textsubscript{1}, R\textsubscript{2}, and R\textsubscript{3} (\Cref{equ:ProjPCM_R1,equ:ProjPCM_R2,equ:ProjPCM_R3}). 
	
	\begin{equation}
		R_{1} = \frac{(R_{ele-PCM} + R_{cryst})\cdot(R_{ele-proj}+R_{proj,c})}{R_{ele-PCM}+R_{cryst}+R_{ele-proj}+R_{proj,c}+R_{int}}
		\label{equ:ProjPCM_R1}
	\end{equation}
	
	\begin{equation}
		R_{2} = \frac{(R_{ele-PCM} + R_{cryst})\cdot R_{int}}{R_{ele-PCM}+R_{cryst}+R_{ele-proj}+R_{proj,c}+R_{int}}
		\label{equ:ProjPCM_R2}
	\end{equation}
	
	\begin{equation}
		R_{3} = \frac{(R_{ele-PCM} + R_{proj,c})\cdot R_{int}}{R_{ele-PCM}+R_{cryst}+R_{ele-proj}+R_{proj,c}+R_{int}}
		\label{equ:ProjPCM_R3}
	\end{equation}
	 
	The total device resistance is given by 
	
	\begin{equation}
		R_{total} = 2 R_1 + \frac{(2 R_2 + R_{amo})\cdot(2 R_3 + R_{proj,a})}{2 R_2 + R_{amo}+2 R_3 + R_{proj,a}}.
		\label{equ:ProjPCM_Rtotal}
	\end{equation}
	
	To gain insights into how the interface resistance influences the state dependence and temporal evolution of the device resistance we employ the device model. Initially, we compare the two most extreme scenarios of zero and infinite \Rint. The material parameters assumed for this calculation are summarized in \Cref{fig:PROJ_Model_ExtremeRinterface}c. The resistance values are chosen such that the typical requirements for CMOS integration in large-scale crossbars are satisfied. For these purposes, the device SET resistance should be on the order of several tens of k$\Omega$ and the maximum RESET resistances close to \unit[1]{M$\Omega$} or larger in order to minimize the ‘IR’ voltage drop on the interconnects which reduces the computational precision when performing in-memory analog computing \cite{Ielmini2018a}. Here, the contact resistances to the metal electrodes are disregarded in order to focus on the effect of the interface resistance between phase change material and projection layer. The contact resistances will be included in the next section for the experimental validation of the model. The drift coefficient associated with the amorphous phase change material, $\nu_R$, is assumed to be 0.1.
	
	First, we study the state dependence of resistance. In the case of no interface resistance (R\textsubscript{int}~=~\unit[0]{$\Omega$}), the device comprises three serial elements of parallel resistors (see \Cref{fig:PROJ_Model_ExtremeRinterface}a). Two are crystalline regions parallel to the projection layer and one is the amorphous region parallel to the projection layer. All resistors in this equivalent circuit scale linearly with the length of the amorphous region in the bridge cell. Thus, the device RESET resistance scales linearly with the amorphous fraction of the device L\textsubscript{amo}/L\textsubscript{line} (blue trace in \Cref{fig:PROJ_Model_ExtremeRinterface}d). In the case of infinite interface resistance (R\textsubscript{int} = \unit[Inf]{$\Omega$}), the device comprises two parallel resistors (\Cref{fig:PROJ_Model_ExtremeRinterface}b). The entire projection layer is parallel to the phase change layer due to the infinite interface resistance. In other words, a fixed resistor (the projection layer) is connected in parallel to a resistor that changes with the amorphous fraction (the phase change layer). Consequently, the device resistance no longer scales linearly with the amorphous fraction as previously observed (red trace \Cref{fig:PROJ_Model_ExtremeRinterface}d).
	
	Next, we study the temporal evolution of device resistance. In a projected PCM device drift deviates from the standard power law for resistance drift $R=R_0 \cdot (t/t_0)^{\nu_R}$ (\Cref{fig:PROJ_Model_ExtremeRinterface}d) irrespective of the amorphous fraction or the interface resistance. The reason is that as the resistance of the amorphous phase increases with time, the current flowing through the amorphous plug decreases, whereas the current flowing through the element \Rproja{} remains constant (assuming a negligible change of the voltage drop over the amorphous segment). Hence over time, the drift suppression in a projected device becomes stronger and the effective drift coefficient time-dependent. The temporal dependence of the drift coefficient is, however, influenced by the interface resistance.
	
	\begin{figure}[bth!]
		\centering
		\includegraphics[width=1\linewidth]{figures/PROJ/Model_ExtremeRinterface.pdf}
		\caption{\textbf{Model assessment for two borderline cases.} \textbf{a}, For the scenario \Rint{} = \unit[0]{$\Omega$}, the projection current bypasses only the amorphous region. \textbf{b}, If \Rint{} is infinite, the projection current must bypass the entire phase change layer. \textbf{c}, Material parameters assumed for the model assessment. R\textsubscript{s} denotes the material sheet resistances. The contact resistance to the electrodes is assumed to be \unit[0]{$\Omega$} to study only the effect of the interface resistance between phase change material and projection layer. \textbf{d}, Device resistance as a function of the amorphous fraction. \textbf{e}, Temporal evolution of the device resistance for different RESET states. \textbf{f}, Drift coefficient one second after programming. Both, device resistance and drift coefficient are sensitive to the interface resistance. In a projected device drift decreases with time (\textbf{e}).}
		\label{fig:PROJ_Model_ExtremeRinterface}
	\end{figure}
	
	In the zero-interface resistance scenario, the resistance ratio between amorphous volume (\Ra) and parallel projection segment (\Rproja) is constant, since both elements scale with L\textsubscript{amo} (\Cref{equ:ProjPCM_Ramo,equ:ProjPCM_Rproja}). The current fraction flowing in the amorphous material, affected by drift, is independent of L\textsubscript{amo}. For small amorphous volumes, when the resistance of the crystalline fraction is non-negligible compared to \Ra$\parallel$\Rproja, the drift coefficient is reduced further. The more the overall device current is determined by the crystalline segment in series with the drifting circuit element (\Ra$\parallel$\Rproja), the less apparent is the effect of drift on the overall device current. Thus, device states with smaller amorphous fractions exhibit a slightly lower effective drift coefficient (blue trace in \Cref{fig:PROJ_Model_ExtremeRinterface}f).
	
	On the other hand, in a device with infinite interface resistance, projection layer and phase change layer are electrically separated. The projecting segment here is constant \linebreak (R\textsubscript{proj}~=~\Rproja~+~\Rprojc~=~\unit[1]{M$\Omega$}). Instead of bypassing only the amorphous volume, the read current must bypass the entire phase change layer. Compared to the zero interface-resistance scenario the fraction of read current flowing in the amorphous volume will always be larger. Moreover, the ratio of current flowing in the projection layer and the phase change layer will be strongly state-dependent. The smaller the amorphous region, the larger the fraction of read current passing through it. Accordingly, smaller amorphous regions lead to a larger effective drift coefficient and drift suppression is worse than in the zero interface-resistance scenario (red trace in \Cref{fig:PROJ_Model_ExtremeRinterface}f).
	
	\subsection{Assessment of model assumptions with FEM simulations}
	
	The device model we propose is an approximate picture of the real device. Our goal is to provide an easily comprehensible and tractable model that is capable to capture key device metrics. Here we address two potential shortcomings of the model. 
	
	First, the field-dependent transport of the amorphous phase is neglected. Hence, the results of our study are valid only in case the device is read in the ohmic regime. In the antimony device studied in this work, we measured an ohmic regime for read voltages smaller than \unit[$\sim$0.15]{V}. For doped \GST{} mushroom cells, ohmic transport has been reported for read voltages smaller than \unit[$\sim$0.2]{V} \cite{Gallo2015}. We assume that it is usually feasible to perform the device read in the ohmic regime. 
	
	Second, we define a localized interface resistor between phase change material and projection layer at the boundary of the crystalline and amorphous phase change material. In reality, the device current will flow from the crystalline material to the projection layer in an extended range around the boundary of crystalline and amorphous phase change material. For metal to semiconductor contacts, this range is defined by the transfer length L\textsubscript{t} = ($\rho$\textsubscript{c}/R\textsubscript{sh})\textsuperscript{0.5}, where $\rho$\textsubscript{c} is the contact resistivity and R\textsubscript{sh} is the sheet resistance of the material from which the current is flowing to another material\cite{Schroder1991}. Accordingly, the material sheet resistances and the interface resistivity determine how localized the current flow from one material to another is. 
	
	The potential error introduced by this model simplification is assessed with 2D FEM simulations (\Cref{fig:PROJ_Model_FEM_study}). The device geometry and material sheet resistances are identical to those defined in \Cref{fig:PROJ_Model_ExtremeRinterface}c. In the FEM model, the current flow between phase change material and projection layer is hindered by the interface resistivity ($\rho$\textsubscript{int}), instead of the localized interface resistance. 
	
	\begin{figure}[bth!]
		\centering
		\includegraphics[width=1\linewidth]{figures/PROJ/FEM_study.pdf}
		\caption{\textbf{FEM vs. Equivalent circuit model. a,} FEM device geometry. The device read is simulated in a 2D model. In the FEM simulation, the spacing of mesh grid points is set to \unit[1]{nm}. \textbf{b}, Current density during read with 100 mV. The interface resistivity between projection layer and phase change material is $\rho$\textsubscript{int} = \unit[0]{$\Omega$\,m\textsuperscript{2}}. The current flow into the projection layer is localized at the crystalline-amorphous interface. \textbf{c},\textbf{d}, Resistance and drift coefficient as a function of the amorphous fraction. FEM simulations are marked by crosses, the equivalent circuit model by full lines. The interface resistance \Rint{} is fitted to match the FEM simulation. All FEM simulations can be reproduced with the simple equivalent circuit model.}
		\label{fig:PROJ_Model_FEM_study}
	\end{figure}
	
	First indications for the soundness of the equivalent circuit model become clear from the simulated current densities (\Cref{fig:PROJ_Model_FEM_study}b). For $\rho$\textsubscript{int} = \unit[0]{$\Omega$\,m\textsuperscript{2}}, i.e. unhindered current flow from the phase change material into the projection layer, the current flow is strongly localized at the crystalline-amorphous interface. 
	
	The equivalent circuit model is further corroborated by comparing the device resistance and drift coefficient as a function of the amorphous fraction with the FEM model. Besides the two scenarios $\rho$\textsubscript{int} \unit[0]{$\Omega$\,m\textsuperscript{2}} and \unit[$\infty$]{$\Omega$\,m\textsuperscript{2}} we also simulate two finite $\rho$\textsubscript{int} (\unit[10\textsuperscript{-9}]{$\Omega$\,m\textsuperscript{2}} and  \unit[10\textsuperscript{-10}]{$\Omega$\,m\textsuperscript{2}}). To identify the corresponding interface resistance, the equivalent circuit model is fitted to the device resistance as a function of the amorphous fraction obtained in the FEM simulation. The only fitting parameter is \Rint. For each $\rho$\textsubscript{int}, a corresponding \Rint{} allows reproducing the scaling of device resistance and drift coefficient with the amorphous fraction (\Cref{fig:PROJ_Model_FEM_study}c\&d). Interestingly, the two models don't match for $\rho$\textsubscript{int} = \unit[0]{$\Omega$\,m\textsuperscript{2}} and \Rint{} = \unit[0]{$\Omega$}. Instead, the FEM simulation with zero-interface resistivity is reproduced with an interface resistance of \unit[55]{k$\Omega$}. The extreme confinement of current flow from the phase change material to the projection layer results in high current densities and current crowding at the interface, leading to a finite effective \Rint.  
	
	We conclude that the distributed interface resistivity in a real device, as well as the current flow from one layer to another over an extended range, can be appropriately described by a localized effective interface resistance located at the boundary between amorphous and crystalline phase change material. However, we acknowledge that the link between material interface resistivity and \Rint{} in our model may be described by a non-trivial functionality, that has not been defined as a part of this work.  

	\subsection{Projected Antimony bridge cell}
	
	In our experimental study, we characterize unprojected and projected bridge cells based on pure Sb. The quantitative assessment of the model should rely on as few unknown fitting parameters as possible. For this reason, the device geometry is inspected by Scanning Transmission Electron Microscopy (STEM) and unprojected bridge cells and thin-film reference structures of the metal nitride are electrically characterized. By this means all model input parameters except for \Rint{} and L\textsubscript{amo} can be obtained in preliminary experiments \Cref{tab:PROJ_ModelParams}. 
	
	\begin{table}[h!]
		\centering
		\begin{tabular}{ c c}
			\hline
			\Rsp{} [k$\Omega$/sq] & 21.8 \\
			\Rsc{} - Sb [k$\Omega$/sq] & 1.26 \\
			\Rsa{} - Sb [k$\Omega$/sq] & 410 $\pm$ 60 \\
			R\textsubscript{W-Sb} [k$\Omega$] & 1.6 \\
			R\textsubscript{W-proj} [k$\Omega$] & 78 to 202 \\ 
			\hline
		\end{tabular}
		\caption{\textbf{Experimentally obtained model input parameters}: The table summarizes the material sheet resistances and contact resistances to the W electrode at an ambient temperature of \unit[200]{K}. The sheet resistance of the amorphous state corresponds to the melt-quenched state one second after device RESET. The contact resistance W to projection material was measured on macroscopic reference structures and extrapolated to the nanoscopic contact area in the device. Accordingly, R\textsubscript{W-proj} is estimated with lower and upper bounds of \unit[78]{k$\Omega$} and \unit[202]{k$\Omega$}, respectively. The errors of the other parameters are negligible, and thus excluded in the analysis.}
		\label{tab:PROJ_ModelParams}
	\end{table}  
	
	In the projected device (\Cref{fig:PROJ_AntimonyDevice}) \unit[6]{nm} metal nitride, functioning as projection material, are added to the initially deposited layer stack (metal nitride, Sb, cladding). It is sputter-deposited without a vacuum break. The subsequent fabrication process is identical to the unprojected bridge cell (see \Cref{Sect:FabricationBridge}) \footnote{Both projected and unprojected bridge cells studied in this chapter have a SiO\textsubscript{2} cladding. The devices studied in \Cref{Chapt:Confine} have a ZnS:SiO\textsubscript{2} cladding instead.}. The cross-section of the \unit[100]{nm} long bridge was investigated by STEM and energy dispersive X-ray spectroscopy (EDX) (\Cref{fig:PROJ_AntimonyDevice}b). In this active region, which is switched between crystalline and amorphous state, the Sb is \unit[45]{nm} wide. The metal nitride stripe underneath is \unit[60]{nm} wide. Differences in the widths of projection and phase change lines result from the mismatch of the etching rates of the phase change and projection layer. During fabrication, the width of the phase change material is reduced by \unit[15]{nm} due to over-etching. For the unprojected device, we measured a width reduction of approximately \unit[8]{nm}, due to over-etching. Note, that a reasonable estimate of the device width is essential to correctly determine the resistors in the equivalent circuit model \footnote{Vara Prasad Jonnalagadda fabricated the devices and prepared TEM lamellas. Marilyne Sousa performed the TEM measurements}. 
	
	\begin{figure}[bth!]
		\centering
		\includegraphics[width=1\linewidth]{figures/PROJ/ProjectedSB.pdf}
		\caption{\textbf{Projected antimony bridge cell. a}, Top view and cross-sectional sketch of the bridge cell with dimensions in nm. HSQ, hydrogen silsesquioxane e-beam resist.  \textbf{b}, STEM and EDX analysis of the active region cross-section along the axis marked in \textbf{a}. The top and bottom panels show an EDX-map for antimony (green) and the metal nitride (orange). These images give an estimate of the bridge width. The central panel is a bright-field STEM image.}
		\label{fig:PROJ_AntimonyDevice}
	\end{figure}
	
	The electrical characterization of the devices is performed at an ambient temperature of \unit[200]{K}, to exclude potential recrystallization of the Sb in our measurements. An estimate for the sheet resistance of the melt-quenched amorphous state (\Rsa -Sb) is obtained from RESET resistances of devices with different bridge lengths (\Cref{fig:PROJ_AntimonySheetResistance}a). It is based on two assumptions about the geometrical constraints of L\textsubscript{amo}. First, we expect that the maximum of L\textsubscript{amo} is defined by the bridge length (i.e. the amorphous volume does not extend beyond the confined region in the device). If the highest RESET resistance measured for the \unit[100]{nm} and \unit[150]{nm} long bridge correspond to a fully amorphous bridge, the sheet resistance would be \unit[350]{k$\Omega$/sq}. This defines the lower limit of \Rsa -Sb.
	Second, we assume that L\textsubscript{amo} of the least resistive RESET state (\unit[74]{k$\Omega$}) is \unit[$\sim$5]{nm}. This corresponds to a sheet resistance of \unit[470]{k$\Omega$/sq}. The amorphous length must be smaller than \unit[6.75]{nm} otherwise the highest resistive RESET states would be larger than the device length. The \unit[74]{k$\Omega$} RESET state is still more than 10x larger than the SET resistance. If L\textsubscript{amo} gets too small, the probability of a crystalline percolation path increases, and consequently, we would expect only a very subtle resistance increase. Based on these considerations \Rsa{} is estimated in the range \unit[410$\pm$60]{k$\Omega$/sq}.
	
	\begin{figure}[tbh!]
		\centering
		\includegraphics[width=1\linewidth]{figures/PROJ/Antimony_SheetResistance.pdf}
		\caption{\textbf{Resistance of amorphous and crystalline Sb: a}, RESET resistance and threshold voltage of devices with different bridge lengths obtained from a series of programming experiments. Both metrics scale linearly with L\textsubscript{amo} \cite{Krebs2009a}. The increase of the achieved RESET resistance with the device length affirms that amorphous volumes of increasing length are created. The bride of these devices is \unit[32]{nm} wide. \textbf{b}, Resistance in the crystalline, pristine device state. Error bars denote the standard deviation measured across multiple devices of the same bridge geometry.}
			
		\label{fig:PROJ_AntimonySheetResistance}
	\end{figure}
	
	The sheet resistance of crystalline Sb is calculated from the pristine resistance of devices with different geometries (\Cref{fig:PROJ_AntimonySheetResistance}b). The device resistance scales linearly with the aspect ratio (length/width) of the bridge. We measure \Rsc - Sb = \unit[1.26]{k$\Omega$/sq} and R\textsubscript{contact} = \unit[1.6]{k$\Omega$}. R\textsubscript{contact} is equivalent to the model parameter R\textsubscript{W-Sb}. It is the sum of the actual contact resistance between the W electrode and Sb and the resistance of the Sb which is not part of the confined bridge; labeled patch in \Cref{fig:PROJ_AntimonyDevice}. Details on the experimental procedure to determine \Rsp, R\textsubscript{W-Sb}, and R\textsubscript{W-proj} are summarized in the Appendix, \Cref{Sect:ProjBridge_preliminary}.  
	
\section{Experimental verification of the model}
	
	In this section drift and RESET resistance of unprojected and projected Sb bridge cells and their dependence on L\textsubscript{amo} are compared. Measurements of the unprojected device provide the last reference points required to fit the characteristics of the projected device to our model. All experiments are performed at \unit[200]{K} ambient temperature.  
	
	\subsection{Drift characterization}
	
	The unprojected bridge cell is programmed to different resistance states with a constant programming current of \unit[610]{$\mu$A} by varying the RESET pulse trailing edge between 3, 5, 7, and \unit[8]{ns}. With increasing pulse trailing edge (duration of melt-quenching process), the RESET resistance decreases, because a larger amount of molten material crystallizes. After programming, the evolution of the resistance as a function of time is measured over \unit[1000]{s} and fitted to the standard drift equation $R=R_0 \cdot (t/t_0)^{\nu_R}$ (\Cref{fig:PROJ_Experiment_Drift}a). We measure a drift coefficient of 0.14 $\pm$ 0.01 for four different intermediate states and find no apparent dependence of the drift coefficient on the pulse trailing edge. Hence, the drift coefficient is independent of the amorphous length. 
	
	\begin{figure}[bth!]
		\centering
		\includegraphics[width=1\linewidth]{figures/PROJ/Experiment_Drift.pdf}
		\caption{\textbf{Drift measurements of unprojected and projected Sb bridge cells}. Different device states were obtained by varying the RESET pulse trailing edge (TE). \textbf{a}, Unprojected cell drift. \textbf{b}, Projected cell drift. Resistance measurements up to \unit[700]{ms} were obtained with an oscilloscope. Measurements from two seconds onward were obtained with a source meter unit. The experimental data are fitted to the device model presented in \Cref{fig:PROJ_DeviceModel}. For both the upper and lower bound of R\textsubscript{W-proj} the model captures the experimental data. \textbf{c}, Fitted parameters: Interface resistance and an individual amorphous length for each RESET state. The error margin is the propagated error of R\textsubscript{s,amo}~-~Sb (\Cref{tab:PROJ_ModelParams}). \textbf{d}, Effective drift coefficient as a function of the amorphous length. The amorphous length of the unprojected cell is calculated for an amorphous sheet resistance of \unit[410]{k$\Omega$/sq}. The drift coefficients measured on unprojected cells (times symbol) are state-independent, whereas the projected cell shows a notable state (plus symbols) and time dependence (\text{b}) of the resistance drift.} 
		\label{fig:PROJ_Experiment_Drift}
	\end{figure}
	
	Compared to the measurements at \unit[100]{K} ambient temperature (\Cref{fig:Nano_Drift_Confinement}) the drift coefficient increases by around 0.04 at \unit[200]{K}. Measurements on a single device at both temperatures confirm that this increase from 0.1 to 0.14 is not an artifact of inter-device variability or different cladding materials in the two studies (ZnS:SiO\textsubscript{2} vs. SiO\textsubscript{2}). In general, the collective relaxation model predicts a temperature-independent resistance drift coefficient (assuming constant temperature during the drift measurement). This has been observed experimentally for ambient temperature in the range from \unit[160]{K} to \unit[420]{K} \cite{LeGallo2018}. However, this statement is only true if the coupling between structural relaxation and electrical conduction does not change. This could happen for example, if the transport mode changes in a certain temperature range (\Cref{Sect:VthDrift_Temperature}) and might be the case here. We observed an Arrhenius temperature dependence between \unit[225]{K} and \unit[175]{K} and a continuous  deviation from this extrapolation with decreasing temperatures for amorphous Sb (\Cref{fig:Nano_PCMcharacteristics}). This change of temperature dependence may indicate a transition to another conduction mode.  

	We now return to the experimental characterization of the projected device. The model predicts a deviation of the resistance drift from the standard relation. Experimentally we measure the time-dependent resistance of four different RESET states (\Cref{fig:PROJ_Experiment_Drift}b). In accordance with the model, the evolution of resistance with time exhibits a clear curvature in the double logarithmic plot. Additionally, the separation between different resistance states decreases with time, indicating a non-zero \Rint{} between the Sb and projection layer.
	
	In order to verify if the device model can capture the measured R(t) data, we attempt to fit it to the model. Having predefined all experimentally directly accessible input parameters (\Cref{tab:PROJ_ModelParams,fig:PROJ_AntimonyDevice}b) and the drift coefficient of antimony, two fit parameters are left to describe the R(t) data of an individual RESET state. Those are \Rint{} between antimony and metal nitride and the L\textsubscript{amo} of the RESET state (\Cref{fig:PROJ_DeviceModel}a). We perform a collective fit of the R(t) traces measured for four different RESET states. The model is able to describe the experiment using a single value of \Rint{} and four different L\textsubscript{amo}. 
	
	Of the experimentally determined model input parameters, the contact resistance R\textsubscript{W-proj} was estimated with the greatest uncertainty. For both the lower and upper bounds of R\textsubscript{W-proj}, the fit captures the experimental data well. The amorphous length obtained from the fit is approximately independent of R\textsubscript{W-proj} (\Cref{fig:PROJ_Experiment_Drift}c). Hence, in the model, the two parameters R\textsubscript{W-proj} and R\textsubscript{int} compensate each other. They determine the fraction of read current that is injected into the projection layer and thus not changed by drift. 
	
	With all model parameters at hand, the state-dependent effective drift coefficient of the projected bridge cell one second after RESET is calculated (\Cref{fig:PROJ_Experiment_Drift}d). Due to the notable \Rint{}, it is comparable to the sheet resistance of the projection layer, the drift exhibits a pronounced state dependence. Depending on the length of the amorphous volume, the drift coefficient is suppressed by a factor of two (for L\textsubscript{amo}~=~\unit[2]{nm}) up to a factor of 10 (for L\textsubscript{amo}~=~\unit[100]{nm}) compared to the unprojected device.
	
	A critical question to answer is if the obtained interface resistance is sensible. To this end, an estimate of the contact resistivity is required. The interface resistance can be described as 
	
	\begin{equation}
		\Rint = \frac{\rho_c}{L_t \cdot w} \cdot coth(L/L_t)
		\label{equ:PROJ_TransferLength}
	\end{equation} 
	
	where $\rho_c$ is the specific contact resistivity, L\textsubscript{t} the transfer length, w the width of the contact area (perpendicular to the direction of current flow), and L the length of the contact area (in direction of current flow) \cite{Schroder1991}. In the bridge cell, L is the length of the contact between crystalline phase change material and projection layer. For the largest amorphous volume (\unit[50]{nm}), the contact between metal nitride and crystalline Sb is \unit[25]{nm} long. Assuming a transfer length of \unit[10]{nm} (i.e. L \textgreater 1.5 L\textsubscript{t}) the interface resistivity in the device can be approximated as $\rho_c = \Rint\cdot w\cdot L_t \approx \unit[50]{k\Omega} \cdot \unit[45]{nm} \cdot \unit[10]{nm} = 2.25\cdot10^{-7} [\Omega\,cm^2]$. Specific contact resistivities in the range \unit[10\textsuperscript{-5} to 10\textsuperscript{-8}]{$\Omega$\,cm\textsuperscript{2}} to metals and metal nitrides have been reported for crystalline \GST{} and GeTe \cite{Cooley2020}. The contact resistance derived in the model fit is well within this range. 
	
	Dedicated contact resistance measurements also show that surface treatment prior to deposition of the phase change material and annealing influence the contact resistance \cite{Cooley2020}. During the device fabrication metal nitride, Sb and cladding were deposited without vacuum break. Subsequent XRR measurements of blanket films indicate a low-density interfacial layer between metal nitride and Sb, which might be attributed to poor adhesion between the two materials. An optimized deposition process could result in better electrical contact and thus improved device characteristics. 
		
	\subsection{Resistance scaling with amorphous volume}
	
	As a second consequence of \Rint, the resistance of the projected device does not scale linearly with the amorphous length. This model prediction is examined experimentally based on the correlation of R\textsubscript{reset} and \Vth{} \footnote{The threshold switching IV characteristics of the projected devices do not exhibit a sharp snap-back point which typically is used as threshold criterion. We observed the same for the unprojected device (\Cref{fig:Nano_PCMcharacteristics}b). For this reason threshold switching is defined as the point where the device current exceeds \unit[12.5]{$\mu$A}. }. In an unprojected bridge cell, the threshold voltage depends linearly on the amorphous length \cite{Krebs2009a}.

	\begin{equation}
		V_{th} = E_{th}\cdot L_{amo} + V_{offset}
		\label{equ:VthGeneral}
	\end{equation}
	
	Here E\textsubscript{th} denotes the threshold field and V\textsubscript{offset} an offset voltage. We expect that this relation is also valid for the projected bridge cell. Switching still occurs at a critical field strength inherent to the phase change material and the field across the amorphous volume is not changed by the electrically parallel projection layer. Accordingly, it should be possible to map R(L\textsubscript{amo}) calculated with the model to the experimental data R(\Vth) using \Cref{equ:VthGeneral}. The best match of the two data sets is obtained for V\textsubscript{th}~=~ \unit[20$\pm$3]{V/$\mu$m} $\cdot$ L\textsubscript{amo} + 0.43 V (\Cref{fig:PROJ_Experiment_ResScaling}). The state dependence predicted with the model is neatly reproduced by the experiment. 
	
	\begin{figure}[bth!]
		\centering
		\includegraphics[width=0.6\linewidth]{figures/PROJ/Experiment_ResScaling.pdf}
		\caption{\textbf{State dependence of RESET resistance in projected Sb bridge cells.} State dependence refers to the dependence of the device resistance on the phase configuration i.e. the amorphous length. Black lines depict the scaling of RESET resistance with the amorphous length predicted by the device model (bottom x-axis). Crosses mark the experimentally obtained data R\textsubscript{RESET} vs V\textsubscript{th} (top x-axis). The linear relation between the top and bottom x-axis is noted in the graph.}
		\label{fig:PROJ_Experiment_ResScaling}
	\end{figure}
	
	The error margin of the threshold field results from the uncertainty of \Rsa{}, and is independent of R\textsubscript{W-Proj}. Notably, we measured the same threshold field on unprojected Sb bridge cells. On the other hand, Krebs et al. report a threshold field of \unit[94$\pm$9]{V/$\mu$m} for as-deposited amorphous Sb (\unit[4]{nm} thick). This discrepancy probably cannot be explained by a more relaxed glass state in the as-deposited amorphous sample. If we assume that threshold switching is induced by a thermal feedback loop \cite{LeGallo2016}, the different temperatures at which the experiments were performed (\unit[200]{K} vs. room temperature) and different slopes of the voltage increase (\unit[1.5]{V}/\unit[60]{ns} vs. "slow" to avoid transient effects \cite{Krebs2010}) could be two hypothetical reasons. De facto a clear answer to the source of the difference cannot be given at this point.  
		
\section{Guidelines for device optimization}
	
	Having validated the proposed device model experimentally, we assess the implications for device applications and the selection of materials for a projected memory device. The state dependence of device drift introduced by a large interface resistance is unfavorable even though the projection layer may reduce the absolute device drift. It cannot be corrected with a global scaling factor. Also a non-linear scaling of RESET resistance with amorphous length may introduce challenges in a device application. The resistance of RESET states with small amorphous lengths changes significantly with the size of the amorphous volume. Thus, it becomes more challenging to program the device to these states. Consequently, only a fraction of the possible device states may be exploited. This could decrease the dynamic resistance range and number of resistance states that can be distinguished reliably.
	
	Even though finite interface resistances pose a challenge to the concept of the projected PCM, within certain bounds they can be tolerated without detrimental effects to the device characteristics. We define three constraints for the device metrics to identify those bounds. First, the maximum drift coefficient should be smaller than 0.01 for amorphous fractions larger than \unit[5]{\%}. In particular, for very small amorphous fractions the drift coefficients increase steeply (\Cref{fig:PROJ_Model_FEM_study}d). We suspect that these are only hypothetical device states in the model and crystalline percolation paths, reducing drift and resistance, would exist in a real device. The \unit[5]{\%} limit is supposed to exclude these states. Second, to restrict drift variability, the resistance separation between the most and least drifting device states must not change by more than \unit[5]{\%} over 4 orders of magnitude in time (\unit[1]{s} to \unit[10\textsuperscript{4}]{s}). We consider this criterion more tangible than a range within which the drift coefficients may vary. Third, the device resistance should deviate for no amorphous fraction by more than \unit[20]{\%} from the linear interpolation between R(amorphous fraction = 0) and R(amorphous fraction = 1). This constraint enforces an approximately linear scaling of the device resistance with L\textsubscript{amo}. 
	
	Here, we study how the maximum interface resistance that can be tolerated to fulfill the aforementioned constraints changes dependent on the ratio of the sheet resistances of projection material, crystalline, and amorphous phase change material (\Cref{fig:PROJ_Model_Extrapolations}a-c). The bridge has an aspect ratio (length/width) of two, the drift coefficient is 0.1 and the contact resistances to the metal electrodes are assumed to be negligible, identical to the initial model assessment (\Cref{fig:PROJ_Model_ExtremeRinterface}c). The curves of the highest interface resistance that allows fulfilling all three criteria can be split into two regimes to the left and right of the maximum. In regime one, at small projection layer resistances, the maximum interface resistance that can be tolerated increases steeply. The projection layer sheet resistance is much smaller than the amorphous sheet resistance. In this case, the constraint enforcing a linear scaling of the device resistance with L\textsubscript{amo} determines the interface resistance. A drift coefficient smaller than 0.01 could also be achieved with large interface resistances. In the second regime, the maximum interface resistance gradually decreases. The limiting constraint is the requirement of a maximum drift coefficient smaller than 0.01. As the projection layer sheet resistance increases and gets closer to the amorphous sheet resistance, the projection must become “better” to suppress the drift sufficiently. A better projection is enabled by a smaller interface resistance. Eventually, the projection layer resistance becomes too large to suppress the drift to 0.01. With increasing ratio of R\textsubscript{s,amo}/R\textsubscript{s,cryst} (\Cref{fig:PROJ_Model_Extrapolations}a–c) the maximum shifts to larger values of R\textsubscript{s,proj}/R\textsubscript{s,cryst} and R\textsubscript{int}/R\textsubscript{s,cryst}. Furthermore, the largest projection layer resistance for which the drift coefficient is smaller than 0.01 increases. Consequently, a larger dynamic range (R\textsubscript{reset}/R\textsubscript{set}) can be realized (color-coded). A high dynamic range is desirable since it allows to write and store the quasi-analog device states with higher precision. Thus, phase change materials with large R\textsubscript{s,amo}/R\textsubscript{s,cryst} are preferable. A projection material and phase change material combination that simply maximizes the tolerable interface resistance is not advantageous. Instead, a compromise between dynamic range and acceptable interface resistance must be made.
	
	\begin{figure}[bth!]
		\centering
		\includegraphics[width=1\linewidth]{figures/PROJ/Model_Extrapolations.pdf}
		\caption{\textbf{Guidelines for device optimization.} Target specifications for future device generations are a drift coefficient smaller than 0.01, a minor state dependence of the drift coefficient, and a close to linear scaling of the resistance with the amorphous length. \textbf{a–c}, The colored area marks feasible projection layer sheet resistances and interface resistances for different ratios \Rsa/\Rsc. The color gradient encodes the dynamic resistance range. \textbf{d}, Estimate of the melt-quenched amorphous to crystalline resistance ratio of different phase change materials. The estimate is obtained from device programming curves. Marker shapes encode the device geometry, compounds of comparable composition are clustered and share a color. (ref. [a,b] - \cite{Yin2007}; [c] - \cite{Zhu2014a}; [d] - \cite{Rao2017}; [e] - \cite{Lankhorst2005}; [f] - \cite{Oosthoek2011}; [g] - \cite{Chen2006}; [h] - \cite{Perniola2010}; [i] - \cite{Bruns2009}; [j] - \cite{Meister2011}; [k] - \cite{Jeyasingh2011}; [l] - \cite{Kim2010a}; [m] - \cite{Jung2006})}
		\label{fig:PROJ_Model_Extrapolations}
	\end{figure}
	
	To assess the suitability of a phase change material for a projected device knowledge of the resistance ratio of the melt-quenched amorphous and the crystalline state is essential. Whilst numerous papers report the resistivity of as-deposited amorphous samples only limited data have been reported for the melt-quenched amorphous phase, the material state of interest in device applications. We use the RESET to SET resistance ratio reported for device programming curves to estimate the resistance ratio of melt-quenched amorphous and crystalline states (\Cref{fig:PROJ_Model_Extrapolations}d). The maximum RESET state created in the programming curves we analyzed appears to be a saturation level, suggesting the size of the amorphous volume has reached a maximum. We note that a saturation of the programming curve does not necessarily correspond to a fully amorphous device. Thus, our analysis may underestimate the materials resistance contrast. 
	
	The studies of doped-SbTe,\cite{Oosthoek2011} and \GST{} \cite{Meister2011,Jeyasingh2011} show TEM figures of an
	amorphized device, suggesting the complete device volume has been amorphized. These two materials and GeTe, all exhibiting resistance ratios larger than 1000, are the most suitable candidates for a projected memory device. However, device studies of highly confined \GST{} \cite{Kim2010a,Jung2006} report a significantly reduced resistance ratio. The programming data reported for N-doped Sb\textsubscript{2}Te\textsubscript{3}, Sc\textsubscript{0.1}Sb\textsubscript{2}Te\textsubscript{3}, and GeSb suggests these materials are not well suited for a projected device. Due to their small resistance ratios (\textless 100) it may be challenging to apply them for a drift and noise resilient multi-level memory devices. For materials with resistance ratios \textless 500 a careful optimization of the projection material, especially the interface resistance, will be required. 
	Since the tolerable \Rint{} scales with \Rsc{}, phase change materials with higher crystalline resistivity would be preferable for a projected device. They would relax the requirements to optimize the contact resistivity between phase change and projection material. Considering there is a certain limit to which the contact resistivity can be reduced this might prove to be another solution. 

\section{Summary \& Outlook}

In a projected memory cell resistance drift is suppressed because only a fraction of the read current flows through the amorphous phase change material. Simulations with the equivalent circuit model we developed and measurements over 7 orders of magnitude in time reveal, that drift becomes time and state-dependent in a projected device. The increasingly stronger drift suppression with time is inherent to the projected memory and can be considered a desirable effect. Whereas the state dependence causes a gradual loss of information with time, that cannot be recovered. Since resistance drift exhibits anyway variability (inter but also intra device), we expect the overall drift reduction by projection still to be beneficial. Furthermore, the drift coefficient becomes only state-dependent if the current flow from the phase change material into the projection layer is hindered. Thus it is critical to minimize the contact resistivity between the two materials. 

Based on the device model a few lessons on how to select projection and phase change material can be learned. First, a drift reduction by 10x implies a reduction of the dynamic range by $\sim$10x, compared to the unprojected device. Additionally, the tolerable interface resistivity can be increased by enlarging the resistance window between the amorphous phase and projection layer (i.e. decreasing \Rsp/\Rsc{}), which would again reduce the dynamic range. Thus the phase change material should have a large dynamic range \Rsc/\Rsa. Second, with increasing resistivity of the phase change material a larger interface resistance (interface resistivity) can be tolerated. This makes phase change materials with higher resistivity preferable. 

As a next step to refine the model and improve its predictive character a more elaborate characterization of \Rint{} is required. In particular, separate measurements of the contact resistivity and transfer length could allow determining \Rint, assuming \Cref{equ:PROJ_TransferLength} can be applied. Potentially another phenomenological description is required. For example due to the device geometry or the metal electrodes which are connected to both materials. Furthermore, we assumed an ohmic contact between projection and crystalline phase change material. If a Schottky barrier forms, \Rint{} to the left and right of the amorphous volume are different. Like in the previous chapter, we identify once again a good understanding of interfacial and confinement effects essential to develop future devices. Besides the implications for phase transition dynamics also those on electronic contacts are critical in a projected memory device. 

Last but not least, we will discuss the transferability of the model to other projected PCM types. Besides the bridge cell, also confined cells and mushroom cells with projection have been studied \cite{Kim2013,Bruce2021,GhaziSarwat2021}. Since the confined cell is basically a vertically flipped bridge cell, the model is applicable to this device type as well. In the mushroom cell (\Cref{fig:Intro_DeviceConcepts}) on the other hand, the geometry of the amorphous volume differs, and, importantly, the phase change material is not in direct contact with the bottom electrode. Projection and phase change material are deposited subsequently, directly on top of the heater. All read current must flow across the interface of the two materials. Furthermore, compared to the crystalline state, the interface resistivity to the amorphous phase change material is typically at least three orders of magnitude larger \cite{Cooley2020}. For this reason, a small interface resistance between projection and crystalline phase change material might be less critical in this device type. Due to the different arrangement of the resistor elements a different equivalent circuit is required to describe this device \cite{GhaziSarwat2021}.

		
\textbf{Key findings:}
\begin{itemize}
	\item	We developed a tractable device model to describe the state and time dependence of drift and how the device resistance scales with the size of the amorphous volume. It captures quantitatively the experiments on projected Sb bridge cells. 
	\item	The time-invariant conduction path in parallel to the drifting amorphous phase change material results in a time-dependent drift coefficient in projected memory cells, irrespective of the device type (mushroom or bridge). The more time elapsed after amorphization, the less the device drifts.  
	\item	Due to the interface resistance between Sb and projection material, the drift coefficient depends also on the size of the amorphous volume. With increasing interface resistance compared to the resistance of the amorphous volume (i.e. decreasing size), less read current bypasses the amorphous phase. The drift coefficient increases for smaller amorphous lengths. By minimizing the contact resistivity between projection layer and phase change material a state-dependent drift coefficient can be avoided. 
\end{itemize}

==> chapters/original1.Relaxation_dynamics.tex <==
\chapter{The origin of structural relaxation}
\label{Chapt:Relax}

\textbf{Preliminary remark:} The results presented in this chapter have been published as journal article. \newline
1) Measurement of onset of structural relaxation in melt-quenched phase change materials - Kersting et al. - Advanced functional materials \cite{Kersting2021} \\[6pt]

When a liquid is quenched faster than its critical cooling rate, crystallization events can be overcome and atoms can structurally freeze into a disordered solid state \cite{Turnbull1969,Zhong2014a,Salinga2018}. Upon cooling the melt, the atomic mobility decreases. Eventually, the system can no longer assume the equilibrium structure of the supercooled liquid state within the timescale of the experiment, and a non-equilibrium glass state is created. The free energy difference between the super-cooled liquid and glass state results in structural relaxation, where the atomic configurations in the glass change over time. The intrinsic material properties, including viscosity, density, and the electronic bandgap, change due to relaxation \cite{Angell2000b,Priestley2005a}, and this is understood to occur in three phases (\Cref{fig:RELA_Sketch3Regimes})\cite{Chen2007,McKenna2003,Priestley2009}. For every rearrangement, a finite energy barrier must be overcome, and therefore, for some amount of time, the onset phase, the properties do not change. In the second phase, where relaxation is most profound, the properties have been observed to change proportionally to log(t). Finally, approaching the supercooled liquid, the glass reaches a saturation phase, and the properties no longer continue to change. 

\begin{figure}[htb]
	\centering
	\includegraphics[width=0.6\linewidth]{figures/RELA/Sketch3Regimes.pdf}
	\caption{\textbf{Sketch of the temporal evolution of material properties upon structural relaxation.} Previous studies of phase change materials have been limited to timescales and temperatures in which drift obeys a log(t) dependence. In this work, we expand the measurement range to the onset of relaxation and study its temperature dependence. Since relaxation is thermally activated, the onset and saturation of drift shift to shorter timescales with increasing ambient temperature.}
	\label{fig:RELA_Sketch3Regimes}
\end{figure}

Tracking this structural relaxation process through all three phases is experimentally challenging. In a PCM device, this might be done by resistance and threshold voltage drift measurements. Although drift has been studied extensively on timescales ranging from hundreds of $\mu$s to \unit[3]{months}, all these experiments only revealed the log(t)-dependency of resistance and threshold voltage \cite{Gorbenko2019,LeGallo2018,Salinga2018,Bruce2021}. A stand-alone sub-\unit[100]{ns} drift measurement by Ielmini et al. on \GST{}  shows a hint of the region where drift is absent \cite{Ielmini2007}. What remains to be investigated both qualitatively and quantitatively are the other two phases, namely, when does structural relaxation begin and when does it end? To this end, measurements that capture the relaxation from extremely short to long timescales at different temperatures are required. 

In the following, we will shed more light on the phase where relaxation is absent. Specifically, we quantify on what timescales the commonly observed log(t)-dependent drift begins. We employ \Vth{} as a means to observe the state of relaxation. The \Vth{} drift of \GST{} mushroom cells is probed at temperatures ranging from \unit[100]{K} to \unit[300]{K} over 9 orders of magnitude in time (tens of ns to \unit[10]{s}). The experimental data are fitted with two models, that have been used to describe structural relaxation and drift in phase change materials, namely the Gibbs model \cite{Gibbs1983,Karpov2007b,Ielmini2008a} and the collective relaxation model \cite{Knoll2009,Sebastian2015,Gallo2016,LeGallo2018}. Finally, we discuss how the collective relaxation model should be modified, if structural relaxation is facilitated by many-body thermal excitations and the consequences of a limited number of structural defects for the relaxation dynamics.  

\section{State of the art}
		
	\subsection{Gibbs relaxation model}
	
	% Gibbs relaxation model
	The relaxation model introduced by Gibbs in the 1980s describes the relaxation process by a spectrum of defect states with different activation energies (q(\Ed)). Each structural defect is described as a double-well potential with activation energy E\textsubscript{d}. Assuming the defect relaxation is thermally activated and obeys a first-order rate equation, the density of defect states changes with time as
	
	\begin{equation}
		\frac{dq(E_\text{d},t)}{dt} = -\nu_0 \cdot \exp\left(\frac{-E_\text{d}}{k_b T}\right) \cdot q(E_\text{d},t).
		\label{equ:RELA_DifferentialGibbs}
	\end{equation}
	
	The attempt to relax frequency $\nu$\textsubscript{0} is estimated on the order of the Debye frequency (\unit[10\textsuperscript{12}]{s\textsuperscript{-1}}) but could change if groups of atoms are involved in a relaxation process \cite{Gibbs1983}. Since the probability to relax depends exponentially on E\textsubscript{d}, defects with small E\textsubscript{d} relax first and only defects in a narrow range of activation energies relax at the same time. The activation energy that must be overcome for further relaxation increases monotonically. 
	
	Structural changes in the material, i.e., the relaxation of defects, reflect on its physical properties (P). The total change is given by 
	
	\begin{equation}
		\Delta P = \int_{0}^{E} c(E_d) \cdot q(E_d)~dE
		\label{equ:RELA_GibbsPropertyChange}
	\end{equation}
	
	with the coupling factor c(E\textsubscript{d}). Only if $\mathrm{c(E_d) \cdot q(E_d)}$ is constant a physical property changes proportional to log(t). In general, the coupling factor could depend on the type of defect or relaxation process \cite{Gibbs1983}. Nevertheless, often times a constant coupling factor between structural relaxation and physical properties is assumed \cite{Friedrichs1989,Shin1993,Khonik2008,Knoll2009}, also in the field of phase change materials \cite{Karpov2007b,Ielmini2008a,LeGallo2018}. Making this assumption, it is possible to derive q(E\textsubscript{d}) from relaxation experiments. In this model, the relaxation onset is determined by the defect states with the lowest E\textsubscript{d} and the finite time it takes to overcome it. The saturation emerges when the super-cooled liquid state is approached. 
	
	Two models, based on these structural relaxation dynamics, have been proposed to describe drift in phase change materials. On the one hand, Karpov et al. assume that the relative volume change (dilatation), affecting \Vth{} and R, is proportional to the number of unrelaxed defect states  \cite{Karpov2007b}. On the other hand, Ielmini et al. argue that the concentration of localized electronic states decreases concomitant with the density of structural defects \cite{Ielmini2007c,Ielmini2008a} (see also \Cref{SubSect:EvolutionBandstructure}). 
	
	The major critique against this relaxation model questions the plausibility of a uniform $\mathrm{c(E_d) \cdot q(E_d)}$ (or $\mathrm{q(E_d)}$, assuming $\mathrm{c(E_d)}$ is constant), necessary to explain the log(t)-dependent change of physical properties \cite{Knoll2009,LeGallo2018}. Interestingly, a wide variety of phenomena in all kinds of glasses can be described by double-well potentials with uniformly distributed activation energies \cite{Karpov2007b}. This might be considered a convenient justification to assume a uniform distribution but by no means provides a physical explanation. Anderson noticed: "Why the statistics of these barriers is so uniform over a wide spectrum of types of glasses remains a mystery" \cite{Anderson1972}. In the context of structural relaxation, it might be explained by the idea that a relaxing defect does not simply vanish but could create new defective configurations with a higher E\textsubscript{d}. Already Gibbs concluded that the activation energy spectrum evolves with time and the spectrum deduced from relaxation measurements includes defects, that arose during the relaxation process \cite{Gibbs1983}. This concept is taken a step further and formulated more explicitly in the collective relaxation model. 
	
	\subsection{Collective relaxation model} 
	
	The collective relaxation model does not specify individual structural defects or relaxation states. Instead, the material is assumed to relax globally towards an ideal glass state \cite{Knoll2009}. With progressing relaxation, the whole system becomes structurally more stabilized. Larger groups or clusters of atoms relax collectively and the activation energy E\textsubscript{b} = E\textsubscript{s}$\cdot$(1-$\Sigma$) of these processes increases monotonically. It depends linearly on the state of relaxation $\Sigma$. $\Sigma$ = 1 is an infinitely unrelaxed state and $\Sigma$\textrightarrow 0 means that the system approaches equilibrium. E\textsubscript{s} is the activation energy as the system approaches equilibrium. Assuming structural transitions 'backward' to a less relaxed state can be neglected, the temporal evolution of the state variable $\Sigma$ is captured in the rate equation
	
	\begin{equation}
		\label{equ:RELA_DifferentialSigma}
		\frac{d\Sigma(t)}{dt}= - \nu_0 \Delta_\Sigma \cdot\exp\left(\frac{-E_\text{s}\cdot(1-\Sigma(t))}{k_\text{b}T}\right).
	\end{equation} 
	
	The attempt to relax frequency $\nu$\textsubscript{0} is expected to be on the order of phonon frequencies and $\Delta$\textsubscript{$\Sigma$} is the change of $\Sigma$ with each relaxation process. Consequently, $\Delta$\textsubscript{$\Sigma$}$\cdot$E\textsubscript{s} defines the increase of the activation energy for each subsequent relaxation step. For a constant ambient temperature, the differential equation can be solved analytically as 
	
	\begin{equation}
		\label{equ:RELA_SigmaOftime}
		\Sigma(t,T) = -\frac{k_\text{b}T}{E_\text{s}} \cdot \log\left(\frac{t+\tau_0}{\tau_1}\right).
	\end{equation}
	
	Here the relaxation onset of the initial glass state $\Sigma_0$  is defined by 
	
	\begin{equation}
		\label{equ:RELA_tau0}
		\tau_0 = \frac{k_\text{b}T}{\nu_0\Delta_\Sigma E_\text{s}} \cdot \exp\left(\frac{E_\text{s}\cdot(1-\Sigma_0)}{k_\text{b}T}\right)
	\end{equation}
	
	and $\mathrm{\tau_1 = \frac{k_\text{b}T}{\nu_0\Delta_\Sigma E_\text{s}} \cdot  \exp(\frac{E_\text{s}}{k_\text{b}T})}$ is the time at which the system reaches equilibrium. In the range $\mathrm{\tau_0<<t<\tau_1}$ the temporal evolution of $\Sigma$ follows log(t) and the change of $\Sigma$ depends linearly on the ambient temperature. 
	
	It is worth noting, that the two models resemble each other and are constructed similarly. In both models, the structural relaxation is described by a first-order rate equation with an Arrhenius temperature dependence on the activation energy. Even though the Gibbs model defines a defect distribution function q(E\textsubscript{d}), at any time the further progress of relaxation is limited by defects with activation energy in a narrow range, and effectively the activation energy of relaxing defects continuously increases, like in the collective relaxation model. 
	
	The defect distribution function of the Gibbs model, however, is a misleading picture. These defect states with different activation energies do not exist at the same time, they are merely an integration over time of the processes that limited the progression of relaxation. We mention once again that already in the 1950s it was conceived that relaxing defects can create new defect states with higher activation energy \cite{Primak1955,Gibbs1983}. The collective relaxation model appears to describe this transition of the system between states with gradually increasing activation energy more naturally.
		
	\subsection{Research questions}
	\begin{enumerate}
		\item	Is it feasible to probe the relaxation onset of a melt-quenched PCM device?
		\item	Can the Gibbs model and the collective relaxation model capture the drift dynamics with time (tens of ns to \unit[10]{s}) and Temperature (\unit[100]{K} to \unit[300]{K})?
		\item	How can the models be challenged further and when/why might they break down?
	\end{enumerate}
	\newpage
	
\section{Threshold voltage drift}
	\label{Sect:VthDrift_Experiment}
	
	Because structural relaxation processes are thermally activated, ambient temperature can be used as a parameter to shift the onset and saturation of drift to experimentally accessible timescales (see \Cref{fig:RELA_Sketch3Regimes}). However, the observation of the saturation phase by raising the ambient temperature (\textgreater \unit[400]{K}) is prohibited due to potential recrystallization of the amorphous phase. On the other hand, there is a potential for measuring the onset of drift by monitoring it at lower ambient temperatures. The challenge, however, is the inability to reliably measure electrical resistance at short-timescales and low temperatures. Hence, we resort to \Vth{} as a means to observe the state of relaxation. 
	
	The study was conducted on \GST{} mushroom cell devices (\Cref{fig:Intro_DeviceConcepts}b), fabricated in the IBM AI hardware center. The multi-layer ring bottom electrode with a radius of $\sim$\unit[20]{nm} and a height of $\sim$\unit[40]{nm} was patterned with a sub-lithographic hardmask process. The sputter-deposited \GST{} film is $\sim$\unit[75]{nm} thick. An on-chip series resistor ($\sim$\unit[2]{k$\Omega$} at \unit[300]{K}), limits the device current at the moment of threshold switching. To assure a stable device operation throughout our study the cells were cycled at least 100,000 times in advance. All experiments presented in this thesis were performed in a JANIS ST-500-2-UHT cryogenic probe station (\Cref{Sect:ProbeStation}). 
	
	The \Vth{} drift is probed, by programming \GST{} mushroom cell devices (\Cref{fig:Intro_DeviceConcepts}b) repeatedly to a new RESET state and applying SET pulses with varying delay times (\Cref{fig:RELA_Experiment_VthDrift}a). The pause t\textsubscript{delay} before applying the SET pulse is increased in logarithmically spaced steps. This sequence with t\textsubscript{delay} ranging from \unit[10]{ns} to \unit[10]{s} is repeated 15 times to average out drift and threshold switching variability. Note that each \Vth{} measurement results in erasure of the corresponding RESET state by recrystallization. The measured \Vth{} drift represents an averaged behavior of RESET states created in the device. Details on the algorithm to define \Vth{} are provided in the Appendix (\Cref{Sect:VthAlgorithm}). 
	
	\subsection{Evolution in three regimes}
	
	\begin{figure}[tbh]
		\centering
		\includegraphics[width=1\linewidth]{figures/RELA/Experiment_VthDrift.pdf}
		\caption{\textbf{Threshold voltage drift experiment. a}, Programming scheme. A RESET pulse with a \unit[3]{ns} falling edge programs the device to a melt-quenched amorphous state. A SET pulse with a \unit[100]{ns} leading edge is applied to probe the threshold voltage value. In the example shown here, the device drifts for \unit[372]{ns} before threshold switching occurs at \unit[1.5]{V}. The time interval (t\textsubscript{delay}) between the RESET and SET pulses is varied to probe the temporal evolution. \textbf{b}, V\textsubscript{th} drift in \GST. The \Vth{} evolution exhibits three distinct regimes (labeled in grey). First a steep increase up to \unit[$\sim$1]{$\mu$s}, second, a flattening to almost constant values, and third a transition to a monotonic increase approximately proportional to log(t).}
		\label{fig:RELA_Experiment_VthDrift}
	\end{figure}
	
	Three distinct regimes are apparent in the temporal evolution of \Vth{}  (\Cref{fig:RELA_Experiment_VthDrift}b). In regime~1, up to \unit[$\sim$1]{$\mu$s}, there is a steep increase of \Vth. This rapid change is most likely caused by the decay of the RESET excitation. On the one hand, a large number of excess charge carriers is generated when the device is molten at high fields, on the other hand, the temperature is locally raised to more than \unit[900]{K} before the applied power is switched off within \unit[3]{ns} (RESET pulse trailing edge). Both a decay of the excess charge carriers \cite{Elliott2020,Ielmini2007} and slow decay of the local temperature when the device is already close to ambient temperature would result in a continuous increase of the threshold voltage. Regime~2 shows a flattening of the curve and almost constant threshold voltage values. Finally, in regime~3 we observe a continuous linear increase with log(t). We attribute the temporal evolution in regimes~2 and 3 to the structural relaxation of the amorphous phase with the transition between them marking the onset of relaxation. 
	
	Careful inspection of the data presented in \cite{Ielmini2007} shows the same three regimes. While a continuous drift with log(t) is observed from about \unit[$\mathrm{10^{-5}}$]{s} in both studies, regime~1 occurs at different timescales. In our study, it lasts up to \unit[1]{$\mu s$} and in the work by Ielmini et al. it ends after approximately \unit[30]{ns}. This could be attributed to the different device geometry and size (mushroom cell with a bottom electrode \unit[$\sim$706]{nm$^2$} vs. $\mu$-trench with a bottom electrode \unit[\textgreater 1500]{nm$^2$}) and the resulting difference in the thermal environment. Additionally, in \cite{Ielmini2007}, the bias of the RESET pulse is reduced to a lower level, sufficient to melt-quench and induce threshold switching, but it is not turned off between RESET and threshold switching. The experiment probes the decay time to a partially excited state (I \unit[$\sim$150]{$\mu$A}) defined by the bias applied at the end of the RESET pulse. Thus, the different bias scheme compared to our experiment, where the bias is completely switched off at the end of the RESET pulse, is another potential reason why regime~1 lasts longer in our study.
	
	In our study, threshold switching is induced by biasing the device with a trapezoidal voltage pulse. \Vth{} changes dependent on the transient signal applied to the device \cite{Wimmer2014a,LeGallo2016}. With decreasing slope of the SET pulse leading edge \Vth{} decreases (\Cref{fig:RELA_Vth_SET_LeadingEdge}a). Both, the electrical stress, and joule heating in the device prior to switching may affect the relaxation dynamics. However, the absolute change of \Vth{} with time appears to be independent of the leading edge (\Cref{fig:RELA_Vth_SET_LeadingEdge}b). This suggests that the rise of the cell bias is fast enough to not notably alter the relaxation process of the glass state, prior to switching. First, the time for which the cell is biased before switching is short on absolute timescales. Second, it is at least in regimes~2 and 3, which are governed by the relaxation dynamics, much shorter than the time for which the material relaxes without any bias being applied.  
	
	\begin{figure}[htb]
		\centering
		\includegraphics[width=1\linewidth]{figures/RELA/Vth_SET_LeadingEdge_v2.pdf}
		\caption{\textbf{Impact of the SET pulse leading edge duration. a}, With an increasing SET pulse leading edge the threshold voltage values decrease continuously. The value of t\textsubscript{drift} is the sum of t\textsubscript{delay} (the delay between the RESET pulse and the SET pulse) and the time elapsed until the applied voltage crosses V\textsubscript{th}. The second term changes with the SET pulse leading edge. The resulting change of t\textsubscript{drift} is most apparent on short timescales, where t\textsubscript{delay} is small. \textbf{b}, The threshold voltage changes with respect to a reference point, which is here the value measured \unit[1]{$\mu$s} after RESET, is independent of the SET pulse leading edge duration. In the legend, the leading edge duration and its slope are noted. All SET pulses have an amplitude of \unit[2.5]{V}.}
		\label{fig:RELA_Vth_SET_LeadingEdge}
	\end{figure}

	\subsection{Temperature-dependent \Vth{} evolution}
	\label{Sect:VthDrift_Temperature}
	
	Next, the threshold voltage evolution with time is probed between \unit[100]{K} and \unit[300]{K} (\Cref{fig:RELA_Tdep_Vth_Drift}). To create comparable RESET states at different ambient temperatures, the programming power was scaled such that the initially molten volume remains approximately constant (\Cref{Sect:SimilarRESETstates}) and the RESET pulse trailing edge was kept constant. This approach is taken to minimize other potential sources of \Vth{} variations and different drift dynamics than the ambient temperature. 
	
	\begin{figure}[htb]
		\centering
		\includegraphics[width=1\linewidth]{figures/RELA/TemperatureDependent_Exp.pdf}
		\caption{\textbf{Temperature-dependent \Vth{} evolution. a}, With decreasing ambient temperature \Vth{} increases. The transient regime~1 is not impacted by temperature. Regime~2, in which \Vth{} reaches a plateau, extends to longer timescales and the drift in regime 3 reduces. \textbf{b}, Threshold voltage change with respect to \unit[1]{$\mu$s}. The evolution with respect to a common reference point highlights the impact of the ambient temperature.}
		\label{fig:RELA_Tdep_Vth_Drift}
	\end{figure}
	
	With increasing ambient temperature, the \Vth{} values decrease. This is due to the thermally activated transport of the amorphous phase. The \Vth{} evolution in regime 1 appears to be almost independent of the ambient temperature (\Cref{fig:RELA_Tdep_Vth_Drift}b). Between \unit[30]{ns} and \unit[1]{$\mu$s} after RESET the threshold voltage increases by \unit[0.4]{V}. Contrary to this, the slope (drift coefficient) in regime 3 decreases at lower ambient temperatures. The transition between regimes 2 and 3, which marks the onset of relaxation changes as well. With decreasing slope in regime 3, it appears to be more gradual and shifted to longer timescales. Both these effects, namely, the onset shift and the slope change are expected because the relaxation processes are decelerated with decreasing temperature.
	
	At \unit[100]{K}, we find \Vth{} drift to be absent, which can be either because the drift coefficient is very small or because the onset has shifted outside of the measurement range. One possible reason for the former might be a change of the transport mode at very low temperatures. In phase change materials with trap states deep within the band gap, like \GST{} \cite{Luckas2010,Rutten2019,Konstantinou2019}, a transition from trap limited band transport to hopping type transport might happen. The activation energy for hopping would be defined by the distance between the Fermi level and the trap states, which may not necessarily change upon structural relaxation. 
	
	\subsection{Relaxation dynamics \& \Vth~drift}
	
	In this subsection, we will try to justify the use of \Vth{} to monitor the state of relaxation, based on experimental observations. Establishing an analytical relation between \Vth{} and the state of relaxation, \Glass, where \Thist{} captures the thermal history, poses a non-trivial problem. First, the exact mechanism of threshold switching is still debated, and second, it is not clear which material parameters change with relaxation. 
	
	We assume that \Vth{} can be defined by the sum of a temperature-dependent function f(T), a term proportional to \Glass{}, and an offset value C\textsubscript{2} that could change with the size of the amorphous dome for example. 
	
	\begin{equation}
		\label{equ:RELA_VariableSeparation}
		V_\text{th} = f(T) + C_1 \cdot \mathrm{Glass}(t,T_{hist}) + C_2
	\end{equation}
	
	A key basis for this assumption is the approximately linear change of V\textsubscript{th} with the activation energy for electrical conduction (E\textsubscript{a}) \cite{Pirovano2004,LeGallo2016}. E\textsubscript{a}, in turn, has been shown to increase with drift \cite{Boniardi2011,LeGallo2018,Wimmer2014b}, and a linear increase of E\textsubscript{a} with log(t) has been experimentally measured for different phase change materials \cite{Fantini2012,Rutten2015}. Thus, we expect that \Vth{} is proportional to \Glass. Finally, we assume that the change of \Vth{} upon relaxation is decoupled from the change with ambient temperature. Such a decoupling was previously deduced in \cite{Ciocchini2012} and \cite{Karpov2007b}. Dependent on the relaxation model, \Glass{} corresponds either to the state variable $\mathrm{\Sigma(t,T_{hist})}$ or the total number of defect states $\mathrm{\int q(E\textsubscript{d},t,T_{hist})~dE}$.  
	
	In the following, we further analyze the temperature-dependent evolution of \Vth{} in regimes 2 and 3. From Equation \ref{equ:RELA_VariableSeparation}, it can be seen that the temporal change in \Vth{} with respect to a defined reference point, $t_\text{ref}$, is dependent only on \Glass, i.e., the state of relaxation. For our analysis, we identify \Vth(1$\mu$s), where drift is absent for all temperatures studied, as an ideal common reference point.  
	
	\begin{equation}
		\label{equ:RELA_DeltVthDeltaGlass}
		\Delta V_\text{th} = V_\text{th}(t,T)-V_\text{th}(1 \mu s,T) = C_1 \cdot (\mathrm{Glass}(t,T_{hist})-\mathrm{Glass_0})
	\end{equation}
	
	We will assume that the initially created, unrelaxed glass state $\mathrm{Glass_0}$ and the coupling factor C\textsubscript{1} do not depend on the ambient temperature. Under this premise, the experiments at all temperatures can be fitted with a common set of parameters.  
		
	\subsection{Model analysis}
	
	The main challenge in probing the Gibbs model is to infer what spectrum of defect states the material has. In fact, experimental studies on other materials show bell-shaped or more complex distribution functions \cite{Shin1993,Chen1976,Tsyplakov2014,Friedrichs1989}. To capture a strict log(t) dependence, however, a rather flat $\mathrm{q(E_\text{d})}$ is required \cite{Gibbs1983,Karpov2007b,Knoll2009}. It has been estimated that the defect spectrum of phase change materials should be constant over more than \unit[0.8]{eV} \cite{LeGallo2018}.
	
	The onset of relaxation is defined by the defects with the smallest activation energy \mbox{(min-E\textsubscript{d})}. How sharp it is, depends on the energy range over which the defect density increases until it becomes rather flat and the attempt to relax frequency. With a wider energy range and smaller frequency, the onset gets stretched out more. Khonic et al. characterized the relaxation onset of a metallic glass (Zr\textsubscript{52.5}Ti\textsubscript{5}Cu\textsubscript{17.9}Ni\textsubscript{14.6}Al\textsubscript{10}) and found an increase of the defect concentration over a range of about \unit[0.5]{eV} (with \nuo{} = \unit[10\textsuperscript{13}]{s\textsuperscript{-1}}) \cite{Khonik2008}. We fit the experiments assuming three different initial defect distributions $\mathrm{q_0(E_\text{d})}$. One with a step-like transition and two with a linear transition over an energy range of \unit[0.25]{eV} and \unit[0.5]{eV} (\Cref{fig:RELA_Gibbs_Collective_Fit}a - Inset). The defect with the highest activation energy is set to \unit[1.5]{eV}, which is well beyond the activation energies that can be overcome on the timescales and temperatures probed in our study. Free fitting parameters are \mbox{min-E\textsubscript{d}}, the attempt to relax frequency \nuo{}, and the coupling factor C\textsubscript{1} (\Cref{tab:RELA_FittingParameters}). 
	
	All three distributions give a fairly good fit. An extrapolation to longer timescales, however, shows that the onset is stretched out too much for the \unit[0.5]{eV} wide transition. The relaxation onset seems to be captured best by a $\mathrm{q_0(E_\text{d})}$ with a sharp transition. During the melt-quenching within nanoseconds, defects with small E\textsubscript{d} can relax. Also, during quenching, the transition between \unit[100]{\%} and \unit[0]{\%} probability to relax is within a narrow energy range at a given time. Thus, it is sensible, that the defect distribution created in the melt-quench process $\mathrm{q_0(E_\text{d})}$ has a sharp transition.  
	
	\begin{figure}[htb]
		\centering
		\includegraphics[width=1\linewidth]{figures/RELA/Gibbs_Collective_Fit.pdf}
		\caption{\textbf{Model fits.} The temporal evolution of V\textsubscript{th} is fitted to (\textbf{a}) Gibbs model and (\textbf{b}) collective relaxation model. \textbf{a}, Three different initial defect distributions (q\textsubscript{0}(E\textsubscript{d}); see inset) are simulated for the Gibbs model. With a widening of the range over which the defect distribution increases the onset gets stretched out more and the relaxation phase (i.e., a constant drift coefficient) is reached later. \textbf{b}, Fit to the collective relaxation model (CR) and the extended model, including the Meyer-Neldel rule (CR+MN). For a better visibility, the experiments at different temperatures are shifted along the y-axis by \mbox{(\unit[T-100]{K})~$\cdot$~\unit[0.2]{V/K}}.}
		\label{fig:RELA_Gibbs_Collective_Fit}
	\end{figure}
	
	Compared to the Gibbs model, the collective relaxation model has fewer degrees of freedom. The initial defect spectrum $\mathrm{q_0(E_\text{d})}$, which gives enough degrees of freedom to notably control or alter the evolution of the relaxation process (e.g., the stretching out of the relaxation onset), is replaced by $\Sigma_0$, a single state variable. By definition, relaxation begins at $\tau_0$ (\Cref{equ:RELA_SigmaOftime}) and subsequently obeys a log(t) dependence. Despite these stricter constraints, the collective relaxation model captures the shift of the relaxation onset to longer timescales and the decrease of the drift coefficient with decreasing ambient temperature neatly (\Cref{fig:RELA_Gibbs_Collective_Fit}b).
	
	In this analysis, four model variables are unknown $\Sigma_0$, C\textsubscript{1}, \Es, and $\nu_0 \Delta_\Sigma$. But since they are interdependent the experiment can be fitted with three parameters (\Cref{tab:RELA_FittingParameters}). The drift coefficient depends on  $\mathrm{C_1/E_s}$ (\Cref{equ:RELA_SigmaOftime,equ:RELA_VariableSeparation}), the exponential prefactor of $\tau_0$ on $\nu_0 \Delta_\Sigma \mathrm{E_s}$ and the exponential term on $\mathrm{(1-\Sigma_0 )\cdot E_s}$ (\Cref{equ:RELA_tau0}). It would be necessary to determine also, when drift saturates ($\tau_1$), in order to obtain the four model variables separately. Based on the fitting parameter  $\mathrm{\nu_0 \Delta_\Sigma E_s}$ and the longest times for which drift has been reported, a lower limit for E\textsubscript{s} can be estimated. In \GST{} drift was measured for more than \unit[8e6]{s} at \unit[300]{K} \cite{Gorbenko2019}. This requires E\textsubscript{s} to be larger than \unit[0.95]{eV}. The upper limit has been estimated on the order of the activation energy for crystallization \cite{LeGallo2018}, which is \unit[3.2]{eV} for \GST{} \cite{Jeyasingh2014a}. 
	
	\begin{table}[htb]
		\centering
		\begin{tabular}{ m{2.2cm} || m{3.5cm} m{3.5cm} m{3.5cm} }
			\toprule[.2em] 
			\multicolumn{4}{c}{} \\
			\multicolumn{4}{c}{Gibbs Model:   $ \frac{dq(E_d,t)}{dt} = -\nu_0 \cdot exp\left(\frac{-E_d}{k_b T}\right)\cdot q(E_d,t)$} \\ 
			\multicolumn{4}{c}{} \\
			\hline \hline
			Transition q\textsubscript{0} & min E\textsubscript{d} [eV] & C\textsubscript{1} [V] & $\nu_0$ [s\textsuperscript{-1}] \\ \hline
			step & 0.16 & -1.57 & 3.66e7 \\
			\unit[0.25]{eV} & 0.12 & -1.54 & 7.33e8 \\
			\unit[0.5]{eV} & 0.05 & -2.33 & 8.64e7 \\
			\midrule[.2em] 
			\multicolumn{4}{c}{} \\
			\multicolumn{4}{c}{Collective relaxation:   $\frac{d\Sigma(t)}{dt}= - \nu_0 \Delta_\Sigma \cdot\exp\left(\frac{-E_\text{s}\cdot(1-\Sigma(t))}{k_\text{b}T}\right)$}\\
			\multicolumn{4}{c}{} \\
			\hline \hline
			& (1-$\Sigma_0$)$\cdot$E\textsubscript{s} [eV] & C\textsubscript{1}/E\textsubscript{s} [V/eV] & $\nu_0\Delta_\Sigma E_s [eV/s]$ \\  \hline
			& 0.19 & -1.2 & 2.48e6 \\
			\midrule[0.2em]
			\multicolumn{4}{c}{} \\
			\multicolumn{4}{c}{Collective relaxation + MN:   $\frac{d\Sigma(t)}{dt}= - \nu_{00}\cdot \exp\left(\frac{-E_\text{s}\cdot(1-\Sigma(t))}{k_\text{b}T_\text{MN}}\right) \Delta_\Sigma \cdot\exp\left(\frac{-E_\text{s}\cdot(1-\Sigma(t))}{k_\text{b}T}\right)$} \\
			\multicolumn{4}{c}{} \\
			\hline \hline
			& (1-$\Sigma_0$)$\cdot$E\textsubscript{s} [eV] & C\textsubscript{1}/E\textsubscript{s} [V/eV] & $\nu_{00}\Delta_\Sigma E_s [eV/s]$ \\ \hline
			& 0.15 & -0.77 & 6.82e4 \\  
			\bottomrule[0.2em]
		\end{tabular}
		\caption{\textbf{Fitting parameters - relaxation models.} The threshold voltage drift is fitted to the Gibbs model, collective relaxation model, and the collective relaxation model including the Meyer-Neldel rule. Comparable model parameters are summarized in the same columns of the table ("smallest activation energy", "coupling factor", "attempt to relax frequency").}
		\label{tab:RELA_FittingParameters}
		
	\end{table}
	
	Interestingly, the relaxation of the glass created at ambient temperatures ranging from \unit[100]{K} to \unit[300]{K} can be fitted with an identical initial glass state $\mathrm{q_0(E_\text{d})}$ and $\Sigma_0$ for Gibbs and Collective relaxation model respectively. The degree of relaxation of the initially created glass state does not notably change. Note, that the relaxation onset $\tau_0$ in the collective relaxation model, depends exponentially on $\Sigma_0$. Variations of the degree of relaxation would have a pronounced impact on $\tau_0$. Faster quenching has been observed to create less relaxed glass states \cite{Greer1982}. In the PCM device, the cooling profile during the melt-quenching process changes with ambient temperature. But seemingly, the part of the cooling profile that defines the initial state of relaxation (it should be defined by the cooling rates at elevated temperatures just below the glass transition temperature), does not change too much. Developing an understanding of the quench rates as well as glass transition temperature in the device and how these determine the initial degree of relaxation could be the subject of future work.    

\section{Discussion}

	Compared to drift measurements in the log(t)-dependent time regime, the value of the here presented experiments lies in the revelation of the deviation from this regime. This new feature of the drift dynamics and in particular its temperature dependence constraints the (effective) attempt to relax frequency (Gibbs: $\nu_0$; collective relaxation: $\nu_0\Delta_\Sigma$) and the lowest defect activation energy (Gibbs: min-\Ed, collective relaxation: \mbox{(1-$\Sigma_0$)\Es)}. It becomes evident in the representation of the onset in the collective relaxation model (\Cref{equ:RELA_tau0}). The linear temperature dependence of $\tau_0$ is almost negligible compared to the exponential term. In a first approximation, the shift of the relaxation onset with temperature is defined by the smallest activation energy for relaxation and the effective attempt to relax frequency is a scaling factor defining the timescale of the onset. 
	
	In both models, the smallest activation energy of defects is on the order of \unit[100]{meV}. In the Gibbs model, it changes slightly depending on the assumed shape of the defect spectrum. In a PCM device, a melt-quenched state is created with extremely high cooling rates on the order of $\sim$\unit[10\textsuperscript{10}]{K\,s\textsuperscript{-1}}. It thus allows studying relaxation from an extremely unrelaxed glass state, which manifests in the low activation energy for relaxation and consequently an onset of relaxation at short timescales.
	
	Previous studies on phase change materials estimated the attempt to relax frequency in the typical phonon frequency range of 10\textsuperscript{13} to \unit[10\textsuperscript{14}]{s\textsuperscript{-1}} \cite{LeGallo2018,Ielmini2008a}. Oftentimes used as a free fitting parameter in the Gibbs model, values ranging from \unit[10\textsuperscript{6}]{s\textsuperscript{-1}} \cite{Stutzmann1986} to \unit[10\textsuperscript{24}]{s\textsuperscript{-1}} \cite{Roura2009} have been reported. We note that these extreme deviations from the typical vibration frequency of atoms in solids are surprising and require further explanation. It has been argued that the attempt frequency may change dependent on the defect activation energy \Ed{} and the number of atoms involved in a relaxation process.  
	
	With increasing \Ed{} the number of possibilities for a transition over \Ed{} increases \cite{Kruger1992}. Yelon et al. described this increase of the 'number of possibilities for a transition' more specifically as the number of ways of assembling excitations (phonons) with total energy \Ed{} \cite{Yelon1992}. This results in an increase of the apparent attempt to relax frequency \nuo{} in accordance with the Meyer-Neldel rule \cite{Meyer1937}. It states that the exponential prefactor (here $\nu_0$) of processes that obey an Arrhenius temperature dependence, increases with \Ed. More precisely ln(\nuo) scales linearly with \Ed. This dependence can be described as $\mathrm{\nu_0 = \nu_{00}\cdot exp(\frac{\Ed}{\kb\TMN})}$, where \TMN{} denotes the Meyer-Neldel temperature and \kb\TMN{} is the energy of a single excitation event (annihilation of a phonon). Taking the Meyer-Neldel rule into account, the fundamental attempt to relax frequency is \nuoo{}, and the apparent attempt to relax frequency \nuo{} might be larger than typical phonon frequencies. 
	
	A decrease of the fundamental attempt to relax frequency \nuoo{} on the other hand has been attributed to configurational changes in large groups of atoms, i.e., cooperative, and hierarchically constrained atomic rearrangements \cite{Kruger1992, Hygate1990, Gibbs1983}. Assume for example a relaxation process that requires 5 randomly vibrating atoms to move in a coordinated way. This coordinated motion may happen at a notably lower frequency than the atomic vibrations. Let us consider the consequence for \nuo{} during relaxation. On the one hand, \Ed{} increases with time, which would cause an increase of \nuo{}. On the other hand, with time larger clusters and groups of atoms may relax collectively, which would result in a decrease of \nuoo{} and counter the increase of \nuo. While the assumption of a constant \nuo{} is a crude approximation, introducing an \Ed{}-dependent spectrum for \nuo{} seems hardly to be possible \cite{Friedrichs1989}, especially since this parameter cannot be measured directly.  
	
	For our analysis, we assumed a constant \nuo, which is on the order of 10\textsuperscript{7} to \unit[10\textsuperscript{8}]{s\textsuperscript{-1}} for the Gibbs model, notably smaller than phonon frequencies. This indicates that the relaxation processes are defined by a cooperative rearrangement of atoms. The corresponding fitting parameter in the collective relaxation models is $\mathrm{\nu_0\Delta_\Sigma E_s}$ = \mbox{\unit[2.46$\cdot$10\textsuperscript{6}]{eV\,s\textsuperscript{-1}}}. The variable $\Delta_\Sigma$ is expected to be $\ll$1; 1/$\Delta_\Sigma$ is the hypothetical number of different configurational states that the system could assume. Accordingly, the collective relaxation model requires orders of magnitude higher attempt to relax frequencies than the Gibbs model. While this is the most striking difference between both models, the general vagueness about the variable makes it difficult to decide if it is an unreasonable value for either of them. 
	
	In the following, we will show how the Meyer-Neldel rule can be implemented in the collective relaxation model and the consequences. Many processes in various materials have been observed to obey the Meyer-Neldel rule. For example, electronic transport \cite{Jackson1988,Overhof1989} as well as defect relaxation in amorphous semiconductors \cite{Crandall1991} and aging in polymers \cite{Crine1991}. Interestingly, Ielmini et al. found that in \GST{} both, relaxation, and crystallization of the glass state, follow the Meyer-Neldel rule with a common \TMN{} = \unit[760]{K} \cite{Ielmini2009}. The same value was later used to model the band gap widening with time \cite{Fantini2012}. 
	
	We incorporate the Meyer-Neldel rule into the collective relaxation model by replacing \nuo{} with $\mathrm{\nu_{00}\cdot exp\left(\frac{(1-\Sigma_0)\Es}{\kb\TMN} \right)}$. With this on the activation energy of the relaxation process dependent attempt to relax frequency, \Cref{equ:RELA_DifferentialSigma} can be rewritten as 
	
	\begin{equation}
		\label{equ:RELA_DifferentialSigma_MN}
		\frac{d\Sigma(t)}{dt}= - \nu_{00} \Delta_\Sigma \cdot\exp\left[\frac{-E_s\cdot(1-\Sigma(t))}{k_b}\cdot\left(\frac{1}{T}-\frac{1}{\TMN}\right)\right].
	\end{equation}
	
	Compared to the version of the model without the Meyer-Neldel rule, \nuo{} is replaced by \nuoo{} and T by $\left(\frac{1}{T}-\frac{1}{\TMN}\right)^{-1}$ in all equations. Note that the Meyer-Neldel rule is only applicable if the activation energy for relaxation is larger than k\textsubscript{b}\TMN = \unit[65]{meV}, i.e., more than one fundamental excitation is required to exceed the energy barrier \cite{Yelon1992}. With (1-$\Sigma_0$)$\cdot$\Es = \unit[190]{meV}, this criterion is met already for the onset of relaxation of the \GST{} device. 
	
	The \Vth{} drift data is fitted to the extended model with \TMN{}~=~\unit[760]{K} (\Cref{fig:RELA_Gibbs_Collective_Fit}b). Within the here studied temperature range both versions of the model capture the experiment. Extrapolated to higher temperatures, however, approaching \TMN, the model predictions begin to deviate notably \Cref{fig:RELA_Impact_MN}. When the Meyer-Neldel rule is taken into account, the drift coefficient increases notably above \unit[300]{K}. With increasing temperature $\tau_0$ decreases less and at around \unit[500]{K} begins to decrease again. Evidently, \Vth{} drift experiments at even higher temperatures could help to probe the validity of the Meyer-Neldel rule further. However, particular care must be taken to exclude a corruption of the drift measurements by gradual recrystallization of the material.   
	
	\begin{figure}[htb]
		\centering
		\includegraphics[width=1\linewidth]{figures/RELA/Impact_MN.pdf}
		\caption{\textbf{Collective relaxation model - impact of the Meyer-Neldel rule. a}, on the threshold voltage drift coefficient and \textbf{b}, on the relaxation onset. The temperature dependence of both parameters is calculated based on the fits to the experiment (\Cref{fig:RELA_Gibbs_Collective_Fit}b \& \Cref{tab:RELA_FittingParameters}). The drift coefficients predicted above \unit[300]{K} deviate notably and $\tau_0$ begins to depart from an Arrhenius temperature dependence when the Meyer-Neldel rule is incorporated in the model.}
		\label{fig:RELA_Impact_MN}
	\end{figure}
		
\section{Gedankenexperiment - a limited number of defects}	
	
	Last but not least we will show in a gedankenexperiment, that drift cannot be explained if one assumes a defined number of structural defects is created during melt-quenching and relaxes/vanishes over time, without creating new defects. 
	
	Studying a map of Switzerland, one notices that only a few main roads through the valleys and over the lowest mountain passes cross the country. All traffic flows along these main connections and falters at the passes. Rizzi et al. nicely discussed that the same picture is valid for the current flow through the amorphous volume in a PCM device. In the disordered state, the activation energy for conduction varies locally and the vast majority of read current will flow through the amorphous volume along a valley with the lowest \Ea{} and be limited by one 'pass' \cite{Rizzi2013}. The idea that effectively only the largest \Ea{} within a conduction path (E\textsubscript{a,limiting}) defines the electrical transport of the amorphous device was also adopted by others \cite{Gallo2015}. A direct consequence of this idea is that drift results mostly from structural rearrangements that alter E\textsubscript{a,limiting}, i.e., relaxation processes in its vicinity. 
	
	Under the premise, that the relaxation of a defect must not create new defects or influence others (i.e., the defect spectrum is created during melt-quenching and does not change) only a limited number of relaxation processes is possible near E\textsubscript{a,limiting}. The rearrangement of one atom in a defective position must reflect on its direct neighbors. Thus, those may not be structural defects in our scenario. Under these constraints, we estimate that the maximum number of structural defects corresponds to \unit[10]{\%} of the atoms in a volume. Let us assume further that the relaxation of defects up to \unit[2]{nm} away from E\textsubscript{a,limiting} can change it. For \GST{} with 9 atoms per unit cell of volume \unit[272]{$\AA^3$} this would correspond to approximately $\frac{4}{3} \pi\cdot 30^3 \cdot \frac{9}{272} = $\unit[3742]{atoms}, surrounding E\textsubscript{a,limiting}, and only \unit[374]{defects}. 
	
	In Monte Carlo simulations we investigate the consequences of a limited number of defects on the relaxation dynamics predicted by the Gibbs model (\Cref{fig:RELA_DefectsFiniteNumber}). In the range from \unit[0.16]{eV} to \unit[1.5]{eV} the defects are distributed uniformly in \unit[10]{meV} bins. Every 1/\nuo{} $\sim$\unit[27]{ns} each defect can relax with the probability $\mathrm{exp\left(\frac{E\textsubscript{d}}{k_bT}\right)}$ (\Cref{tab:RELA_FittingParameters,equ:RELA_DifferentialGibbs}). With decreasing number of defects, the temporal evolution becomes less smooth. If the initial spectrum is made up of less than $\sim$1000 defects, the defect evolution begins to exhibit discontinuities. In a resistance drift measurement, this would manifest in jump-like increases of the device resistance. To our best knowledge, no indications for such discontinuities have been observed. Admittedly, they might be hidden by the device read noise. 
	
	\begin{figure}[hbt]
		\centering
		\includegraphics[width=0.6\linewidth]{figures/RELA/Simulate_FiniteNumberOfDefects.pdf}
		\caption{\textbf{Monte Carlo Simulation - finite number of defects.} The defect relaxation is simulated for different total numbers of defects. With decreasing number of defects, the relaxation dynamics become increasingly stochastic and begin to scatter around the behavior of a system with many defects. For these simulations, the parameters obtained with the Gibbs model for a uniform defect distribution were used (\Cref{tab:RELA_FittingParameters}).}
		\label{fig:RELA_DefectsFiniteNumber}
	\end{figure}
	
	Altogether this picture of a defined number of defects that vanish with time seems odd. And even though we assume the relaxation of defects in fairly large volume results in an increase of E\textsubscript{a,limiting}, the Monte Carlo simulations indicate jump-like increases of the resistance during drift. It provides further evidence, that the defect spectrum used in the Gibbs model does not exist at any time but is an integration, of the defects limiting the progression of structural relaxation, over time. The rearrangement of a defective configuration results in another, energetically more favorable defective configuration, which has larger activation energy for relaxation. Like this multiple relaxation processes can occur in one and the same spot within the material, specifically where E\textsubscript{a,limiting} is located. Apparently, the conceptual idea behind the collective relaxation model describes the relaxation process more naturally.  
	
\section{Summary \& Outlook}

The evolution of \Vth{}, between \unit[$\sim$30]{ns} and \unit[10]{s} after melt-quenching the device, exhibits three distinct regimes. Initially, within the first $\mu$s \Vth{} increases steeply, next the value stagnates and finally begins to increase again proportional to log(t). We attribute regime 1 to the decay of the RESET excitation (electronic and/or thermally) and identify the dynamics of structural relaxation as the cause of regimes 2 and 3. The shift of the transition between these regimes with temperature is captured by the Gibbs model and the collective relaxation model. We note that the excellent match between experimental data and the models can be considered another indication that drift in phase change materials must be attributed to structural relaxation.  

With respect to the first two research questions, we can state. Yes, it is feasible to probe the onset of relaxation in a PCM device by \Vth{} measurements. No, the relaxation models alone cannot capture the full experiment, but only the time-evolution beginning from one $\mu$s. On shorter timescales other effects, most likely the transient decay of the RESET excitation must be taken into account. This phenomenon requires further investigation. It might be of particular importance when read and write operations are executed within nanoseconds, i.e., on an integrated chip with a clock in the MHz range.

Regarding the limitations and potential shortcomings of the Gibbs model, it should be noted that a uniform defect distribution appears to capture the experiments best. The sensibility of such a distribution, in particular across all kinds of materials exhibiting a log(t)-dependent change of their physical properties, has been questioned frequently. Additionally, our Monte Carlo simulations of a system with a fixed number of defects show that in this scenario resistance drift would probably exhibit step-like jumps. We conclude that the relaxation of one defect must be expected to create new defects that relax later. The defect spectrum used in the Gibbs model to describe the relaxation does not exist at any time but is actually the result of an integration of defects that limit the further progress of relaxation over time.

Last but not least, it should be noted that both relaxation models must be modified if structural relaxation is facilitated by many-body thermal excitation. Here, we discussed the implications for the collective relaxation model. Within the studied temperature range, both versions of the model capture the experiments with subtle differences. At even higher temperatures $\sim$\unit[350]{K} and above, however, the model predictions begin to deviate. As k\textsubscript{b}T approaches the energy of a single excitation process, the modified model predicts a significantly larger $\nu$\textsubscript{Vth} and a weaker temperature dependence of $\tau_0$. As long as the phase change material does not begin to crystallize, drift measurement at higher temperatures could allow differentiating which model prediction is correct; an essential step to identifying a model that allows simulating reliably the impact of time, but also temperature variations on \Vth{} and device resistance.  






\textbf{Key findings:}
\begin{itemize}
	\item	In a \GST{} mushroom cell, the onset of structural relaxation is around \unit[$\sim$15]{$\mu$s} after melt-quenching the device, at \unit[300]{K} ambient Temperature. At this time, defects with activation energy on the order of \unit[150]{meV} begin to relax. 
	
	\item	Assuming a fixed, finite number of defect states is created during melt-quenching and vanishes upon relaxation cannot plausibly explain drift in phase change materials. Instead, the relaxation of a structural defect must be expected to result in another defective configuration that can relax further. The collective relaxation model is motivated by this very idea. In this regard, the defect distribution defined in the Gibbs model is misleading. 
	
	\item	We have shown how the Meyer-Neldel rule can be incorporated into the collective relaxation model. If structural relaxation is enabled by thermal many-body excitations, as other studies indicate, this refined model should be used to describe drift. Both versions of the model capture the experimental data, but for higher ambient temperatures the model predictions begin to deviate notably. 
	
\end{itemize}
	
	

==> chapters/outdated/Phase_change_memory_devices.tex <==
\chapter{Phase change memory devices}




\begin{itemize}
	\item	define SET \& RESET; phase transition amorphous / crystalline 
	\item	locally heat to ~1000 K	
\end{itemize}

\section{Device concepts}

	\begin{itemize}
		\item	confined material
		\item	confined electrodes
	\end{itemize}

\section{Principles of device operation}

	\begin{itemize}
		\item 	SET state IV characteristic
		\item 	RESET state IV characteristic
		\item	Programming curve
		\item	SET window 
	\end{itemize}

\section{Device non-idealities}

	\begin{itemize}
		\item 	Wake-Up effects
		\item	Drift
		\item	Read noise
		\item	Activated transport
		\item	Stochasticity
	\end{itemize}




==> chapters/outdated/b02-abstract.tex <==
%\chapter*{Abstract}


==> chapters/outdated/b03-affidavit.tex <==
\chapter*{Eidesstattliche Erklärung}

Hiermit versichere ich, \textit{Vorname Nachname}, dass ich die vorliegende Arbeit selbstständig verfasst und keine anderen als die angegebenen Quellen und Hilfsmittel verwendet habe. Gedanklich, inhaltlich oder wörtlich übernommenes habe ich durch Angabe von Herkunft und Text oder Anmerkung belegt bzw. kenntlich gemacht. Dies gilt in gleicher Weise für Bilder, Tabellen, Zeichnungen und Skizzen, die nicht von mir selbst erstellt wurden.

%Alle auf der CD beigefügten Programme sind von mir selbst programmiert worden.

\par
\vspace*{10ex}

\begin{minipage}[b][][t]{0.5\textwidth}
	Münster, 29. September 2015
\end{minipage}
\hfill
\begin{minipage}[b][][b]{0.5\textwidth}
	\hrulefill
\end{minipage}

\par
\vspace*{-2ex}
\hfill
\begin{minipage}{0.5\textwidth}
	\centering
	Vorname Nachname
\end{minipage}

==> chapters/outdated/b04-acknowledgement.tex <==
%\chapter*{Acknowlegement}
